Controllable Dynamic Multi-Task Architectures

Multi-task learning commonly encounters competition for resources among tasks, specifically when model capacity is limited. This challenge motivates models which allow control over the relative importance of tasks and total compute cost during inference time. In this work, we propose such a controllable multi-task network that dynamically adjusts its architecture and weights to match the desired task preference as well as the resource constraints. In contrast to the existing dynamic multi-task approaches that adjust only the weights within a fixed architecture, our approach affords the flexibility to dynamically control the total computational cost and match the user-preferred task importance better. We propose a disentangled training of two hypernetworks, by exploiting task affinity and a novel branching regularized loss, to take input preferences and accordingly predict tree-structured models with adapted weights. Experiments on three multi-task benchmarks, namely PASCAL-Context, NYU-v2, and CIFAR-100, show the efficacy of our approach. Project page is available at https://www.nec-labs.com/~mas/DYMU.

==> plots/nyu/nyu_marginals_pgfplot.tex <==
\begin{figure*}
  \centering\centering
  \begin{subfigure}{0.32\linewidth}
%
\begin{tikzpicture}[
    thick,
    >=stealth',
    dot/.style = {
      draw,
      fill = white,
      circle,
      inner sep = 0pt,
      minimum size = 4pt
    }
]
\begin{axis}[
    width=5.8cm,
    height=4cm,
    grid=major,
    major grid style={line width=.2pt,draw=gray!50},
    xmin=0,
    xmax=1.0,
    ymin=1.35,
    ymax=3.25,
    axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.5,-0.15)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},rotate=90,anchor=south},
    y tick label style={
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=1,
    /tikz/.cd
    },
    xlabel={Task preference},
    ylabel={Loss},
    legend style={at={(0.45, 0.8)}, anchor=west, draw=none},
    legend cell align={left},
]
\addplot[color=orange,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 3.15)
    (0.3, 2.22)
    (0.5, 1.69)
    (0.7, 1.52)
    (0.9, 1.51)
};
\addplot[color=cyan,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 2.94)
    (0.3, 1.65)
    (0.5, 1.57)
    (0.7, 1.52)
    (0.9, 1.51)
};
\addplot[color=orange,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.86)
    (0.3, 1.50)
    (0.5, 1.59)
    (0.7, 1.62)
    (0.9, 1.62)
};
\addplot[color=cyan,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.72)
    (0.3, 1.54)
    (0.5, 1.60)
    (0.7, 1.63)
    (0.9, 1.60)
};
\end{axis}
\end{tikzpicture} 
%
    \caption{Semantic Segmentation}
    \label{fig:nyu_marginal_semseg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.32\linewidth}
%
\begin{tikzpicture}[
    thick,
    >=stealth',
    dot/.style = {
      draw,
      fill = white,
      circle,
      inner sep = 0pt,
      minimum size = 4pt
    }
]
\begin{axis}[
    width=5.8cm,
    height=4cm,
    grid=major,
    major grid style={line width=.2pt,draw=gray!50},
    xmin=0,
    xmax=1.0,
    ymin=1.9,
    ymax=4.5,
    axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.5,-0.15)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},rotate=90,anchor=south},
    y tick label style={
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=1,
    /tikz/.cd
    },
    xlabel={Task preference},
    ylabel={Loss},
    legend style={at={(0.45, 0.8)}, anchor=west, draw=none},
    legend cell align={left},
]
\addplot[color=orange,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 4.32)
    (0.3, 2.81)
    (0.5, 2.28)
    (0.7, 2.11)
    (0.9, 2.06)
};
\addplot[color=cyan,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 4.27)
    (0.3, 2.31)
    (0.5, 2.18)
    (0.7, 2.12)
    (0.9, 2.06)
};
\addplot[color=orange,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 3.11)
    (0.3, 2.48)
    (0.5, 2.09)
    (0.7, 2.07)
    (0.9, 2.05)
};
\addplot[color=cyan,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 3.33)
    (0.3, 2.32)
    (0.5, 2.06)
    (0.7, 2.05)
    (0.9, 2.04)
};
\end{axis}
\end{tikzpicture} 
%
    \caption{Surface Normals}
    \label{fig:nyu_marginal_normals}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.32\linewidth}
%
\begin{tikzpicture}[
    thick,
    >=stealth',
    dot/.style = {
      draw,
      fill = white,
      circle,
      inner sep = 0pt,
      minimum size = 4pt
    }
]
\begin{axis}[
    width=5.8cm,
    height=4cm,
    grid=major,
    major grid style={line width=.2pt,draw=gray!50},
    xmin=0,
    xmax=1.0,
    ymin=1.15,
    ymax=2.9,
    axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.5,-0.15)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},rotate=90,anchor=south},
    y tick label style={
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=1,
    /tikz/.cd
    },
    xlabel={Task preference},
    ylabel={Loss},
    legend style={
    at={(1.06, 1.0)},
    anchor=north east,
    draw=none
    },
    legend cell align={left},
]
\addplot[color=cyan,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 2.52)
    (0.3, 1.39)
    (0.5, 1.36)
    (0.7, 1.33)
    (0.9, 1.32)
};
\addlegendentry{$c=0.0$};
\addplot[color=orange,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 2.87)
    (0.3, 1.43)
    (0.5, 1.38)
    (0.7, 1.33)
    (0.9, 1.32)
};
\addlegendentry{$c=1.0$};
\addplot[color=cyan,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.75)
    (0.3, 1.31)
    (0.5, 1.30)
    (0.7, 1.29)
    (0.9, 1.28)
};
\addlegendentry{$c=0.0$ (w/ adaptation)};
\addplot[color=orange,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.82)
    (0.3, 1.30)
    (0.5, 1.30)
    (0.7, 1.29)
    (0.9, 1.29)
};
\addlegendentry{$c=1.0$ (w/ adaptation)};
\end{axis}
\end{tikzpicture} 
%
    \caption{Depth}
    \label{fig:nyu_marginal_depth}
  \end{subfigure}
  \vspace{-0.25cm}
  \caption{\textbf{Marginal evaluation of tasks on NYU-v2}}
  \label{fig:marginal_nyu}
\end{figure*}

==> plots/pascal3/pascal3_marginals_pgf.tex <==
\begin{figure*}
  \centering\centering
  \begin{subfigure}{0.32\linewidth}
%
\begin{tikzpicture}[
    thick,
    >=stealth',
    dot/.style = {
      draw,
      fill = white,
      circle,
      inner sep = 0pt,
      minimum size = 4pt
    }
]
\begin{axis}[
    width=5.8cm,
    height=4cm,
    grid=major,
    major grid style={line width=.2pt,draw=gray!50},
    xmin=0,
    xmax=1.0,
    ymin=0.25,
    ymax=1.5,
    axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.5,-0.15)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},rotate=90,anchor=south},
    y tick label style={
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=1,
    /tikz/.cd
    },
    xlabel={Task preference},
    ylabel={Loss},
    legend style={at={(0.45, 0.8)}, anchor=west, draw=none},
    legend cell align={left},
]
\addplot[color=orange,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.44)
    (0.3, 0.56)
    (0.5, 0.36)
    (0.7, 0.34)
    (0.9, 0.32)
};
\addplot[color=cyan,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.39)
    (0.3, 0.51)
    (0.5, 0.35)
    (0.7, 0.34)
    (0.9, 0.32)
};
\addplot[color=orange,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.02)
    (0.3, 0.35)
    (0.5, 0.33)
    (0.7, 0.33)
    (0.9, 0.32)
};
\addplot[color=cyan,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.01)
    (0.3, 0.35)
    (0.5, 0.33)
    (0.7, 0.32)
    (0.9, 0.32)
};
\end{axis}
\end{tikzpicture} 
%
    \caption{Semantic Segmentation}
    \label{fig:pascal3_marginal_semseg}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.32\linewidth}
%
\begin{tikzpicture}[
    thick,
    >=stealth',
    dot/.style = {
      draw,
      fill = white,
      circle,
      inner sep = 0pt,
      minimum size = 4pt
    }
]
\begin{axis}[
    width=5.8cm,
    height=4cm,
    grid=major,
    major grid style={line width=.2pt,draw=gray!50},
    xmin=0,
    xmax=1.0,
    ymin=0.35,
    ymax=1.5,
    axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.5,-0.15)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},rotate=90,anchor=south},
    y tick label style={
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=1,
    /tikz/.cd
    },
    xlabel={Task preference},
    ylabel={Loss},
    legend style={at={(0.45, 0.8)}, anchor=west, draw=none},
    legend cell align={left},
]
\addplot[color=orange,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.48)
    (0.3, 0.83)
    (0.5, 0.77)
    (0.7, 0.51)
    (0.9, 0.51)
};
\addplot[color=cyan,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.47)
    (0.3, 0.83)
    (0.5, 0.73)
    (0.7, 0.51)
    (0.9, 0.50)
};
\addplot[color=orange,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 0.81)
    (0.3, 0.58)
    (0.5, 0.53)
    (0.7, 0.49)
    (0.9, 0.49)
};
\addplot[color=cyan,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 0.81)
    (0.3, 0.57)
    (0.5, 0.53)
    (0.7, 0.49)
    (0.9, 0.47)
};
\end{axis}
\end{tikzpicture} 
%
    \caption{Human Parts}
    \label{fig:pascal3_marginal_parts}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.32\linewidth}
%
\begin{tikzpicture}[
    thick,
    >=stealth',
    dot/.style = {
      draw,
      fill = white,
      circle,
      inner sep = 0pt,
      minimum size = 4pt
    }
]
\begin{axis}[
    width=5.8cm,
    height=4cm,
    grid=major,
    major grid style={line width=.2pt,draw=gray!50},
    xmin=0,
    xmax=1.0,
    ymin=0.2,
    ymax=1.75,
    axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.5,-0.15)},anchor=north},
    y label style={at={(axis description cs:-0.15,.5)},rotate=90,anchor=south},
    y tick label style={
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=1,
    /tikz/.cd
    },
    xlabel={Task preference},
    ylabel={Loss},
    legend style={
    at={(1.06, 1.0)},
    anchor=north east,
    draw=none
    },
    legend cell align={left},
]
\addplot[color=cyan,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.62)
    (0.3, 0.55)
    (0.5, 0.42)
    (0.7, 0.35)
    (0.9, 0.34)
};
\addlegendentry{$c=0.0$};
\addplot[color=orange,solid,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 1.62)
    (0.3, 0.88)
    (0.5, 0.41)
    (0.7, 0.35)
    (0.9, 0.34)
};
\addlegendentry{$c=1.0$};
\addplot[color=cyan,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 0.48)
    (0.3, 0.33)
    (0.5, 0.32)
    (0.7, 0.31)
    (0.9, 0.31)
};
\addlegendentry{$c=0.0$ (w/ adaptation)};
\addplot[color=orange,dashed,thick,mark=*, mark options={fill=white,solid}] coordinates {
    (0.1, 0.48)
    (0.3, 0.36)
    (0.5, 0.32)
    (0.7, 0.31)
    (0.9, 0.31)
};
\addlegendentry{$c=1.0$ (w/ adaptation)};
\end{axis}
\end{tikzpicture} 
%
    \caption{Saliency}
    \label{fig:pascal3_marginal_sal}
  \end{subfigure}
  \vspace{-0.25cm}
  \caption{\textbf{Marginal evaluation of tasks on PASCAL-Context (3 tasks)}}
  \label{fig:marginal_pascal3}
\end{figure*}

==> sections/experiments.tex <==
% \newpage
\section{Experiments}
\iffalse
In this section, we demonstrate the ability of our framework to dynamically search for compact architectures for efficient multi-task learning. Extensive experiments show that the predicted network structures are diverse and match well with the input preferences, in terms of both resource usage and task performance.
% \YM{Explicitly say that Single-Task (=multiple single-task networks) is another baseline, i.e., the other extreme of weight-only hypernet: Single Task (high acc, low compute eff) -- PHN-BN (low acc, high compute eff))
% 1) ours is flexible between two extremes (in terms of both HV and compute cost)
% 2) sometimes even perform better than Single Task with lower compute cost}
\fi
In this section, we demonstrate the ability of our framework to dynamically search for efficient architectures for multi-task learning. We show that our framework achieves flexibility between two extremes of the accuracy-efficiency trade-off, allowing a better control within a single model. Extensive experiments indicate that the predicted network structures match well with the input preferences, in terms of both resource usage and task performance.
% \YM{diverse?}
% \vskip 4pt
% \noindent \textbf{Evaluation Criteria.} 
\subsection{Evaluation Criteria}
\noindent \textbf{Uniformity.}
To measure controllability with respect to task preferences, we utilize uniformity~\cite{mahapatra2020multi} which quantifies how well the vector of task losses $\bm{L} = [\mathcal{L}_1,\dots,\mathcal{L}_N]$ is aligned with the given preference. Specifically, for the loss vector $\bm{L}$ corresponding to the architecture for task preference $\bm{r}$, uniformity is defined as $\mu_{\bm{r}} = 1 - \infdiv{\hat{\bm{L}}}{\bm{1}/N}$, where $\hat{\bm{L}}(j) = \frac{r_j\mathcal{L}_j}{\sum_i r_i\mathcal{L}_i}$. This arises from the fact that, ideally, $r_j \propto 1/\mathcal{L}_j$, which in turn implies $r_1\mathcal{L}_1=r_2\mathcal{L}_2\dots=r_N\mathcal{L}_N$. 
% We also measure the controllability with respect to the resource preference $c$ by evaluating the ratio of the average size of the predicted architectures to the size of the full anchor net.
% \vskip 2pt

\noindent \textbf{Hypervolume.}
Using the trained controller, we are able to approximate the trade-off curve among the different tasks in the loss space. To evaluate the quality of this curve, we utilize hypervolume (HV)~\cite{zitzler1999multiobjective} -- a popular metric in the multi-objective optimization literature to compare different sets of solutions approximating the Pareto front \cite{fleischer2003measure}. It measures the volume in the loss space of points dominated by a solution in the evaluated set. Since this volume is unbounded, hypervolume measures the volume in a rectangle defined by the solutions and a selected \emph{reference point}. More details can be found in the supplementary.
% \vskip 2pt

\noindent \textbf{Computational Resource.}
We measure the computational cost using the memory of the activated nodes in the anchor net and the GFLOPs, which approximates the time spent in the forward pass.
% proportional to the computational cost spent in the forward pass and approximates the inference time.
We also report the computational cost of the hypernets to take into account their overheads. 
%Note that this overhead will materialize only when the preference changes and does not have any effect on the task inference.
% sparsely occur in practical scenarios, only when the preference changes.
We discuss more on the model size in the supplementary document.
% In this work, we consider inference time as a measure of computational resource. We believe fast inference matters in many practical scenarios, whereas reasonable amount of increase in memory overhead is relatively easy to handle. This justifies our design choice to introduce the anchor net.
% \vskip 4pt
% \noindent \textbf{Datasets.}
\subsection{Datasets}
We evaluate the performance of our approach using three multi-task datasets, namely \textbf{PASCAL-Context}~\cite{mottaghi2014the} and \textbf{NYU-v2}~\cite{silberman2012indoor}, and \textbf{CIFAR-100}~\cite{krizhevsky2009learning}. The PASCAL-Context dataset is used for joint semantic segmentation, human parts segmentation and saliency estimation, as well as these three tasks together with surface normal estimation, and edge detection as in \cite{bruggemann2020automated}. The NYU-v2 dataset comprises images of indoor scenes, fully labeled for semantic segmentation, depth estimation and surface normal estimation. For CIFAR-100, we split the dataset into 20 five-way classification tasks~\cite{rosenbaum2017routing}.
% \YM{Comparison with Controllable for 20 tasks CIFAR100?}
% \vskip 4pt
% \noindent \textbf{Baselines.}
%\input{plots/nyu/nyu_marginals_pgfplot}
%\input{plots/pascal3/pascal3_marginals_pgf}
\subsection{Baselines}
We compare our framework with both \emph{static} and \emph{dynamic} networks. Static networks include \textbf{Single-task} networks, where we train each task separately using a task-specific backbone, and \textbf{Multi-task} networks, in which all tasks share the backbone but have separate task-specific heads at the end. These multi-task networks are trained separately for different preferences and thus, training time scales linearly with the number of preferences. We use this to contrast the training time of our framework. The single-task networks demonstrate the anchor net performance. We also compare our architectures with two multi-task NAS methods, \textbf{LTB}~\cite{li2020learning} and \textbf{BMTAS}~\cite{bruggemann2020automated}, which use the same tree-structured search space to perform NAS, but are static. The dynamic networks include Pareto Hypernetworks (\textbf{PHN}) \cite{navon2021learning}, which  predicts only the weights of a shared backbone network conditioned on a task preference vector using hypernetworks, and \textbf{PHN-BN}, a variation of PHN which predicts only the normalization parameters similar to our weight hypernet. Implementation details are presented in the supplementary.
% We use the same backbone and task-specific heads for all methods (including our proposed approach) for a fair comparison. 
%\begin{figure}
%\centering
%
%\begin{subfigure}[b]{0.4\textwidth}
%\includegraphics[width=\linewidth]{plots/nyu/nyu_hv.pdf}
%\caption{}
%\label{fig:nyu_hv}
%\end{subfigure}
%
%\begin{subfigure}[b]{0.4\textwidth}
%\includegraphics[width=\linewidth]{plots/pascal3/pascal3_hv.pdf}
%\caption{}
%\label{fig:pascal3_hv}
%\end{subfigure}
%
%\caption{\textbf{HV multitask}}
%\label{fig:multitask_hv}
%\end{figure}

% \MC{The following paragraph has a few different threads. Make ``Comparison with Baselines'' a sub-section and have separate paragraphs for each. Group the remaining paragraphs as something like ``Analysis of Controllability''.}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{plots/nyu/cost_main.pdf}
    \vspace{-0.2cm}
    \caption{\textbf{Resource usage on NYU-v2.} We visualize resource usage by plotting the proportion of parameters active in the anchor net versus the task preference. The three vertices represent the task preferences with non-zero importance to only one task, while areas in the middle correspond to more dense preferences. As $c$ increases, the predicted networks grow progressively smaller in the dense regions. On the other hand, conventional dynamic networks for MTL always have a constant resource usage ($\mathcal{T}_1$:semantic seg., $\mathcal{T}_2$:surface normal, $\mathcal{T}_3$:depth).}
    \label{fig:resource}
    \vspace{-0.5cm}
\end{figure}

\subsection{Comparison with Baselines}

% \begin{itemize}
%     \item Resource usage comparison (add baseline to current Figure 8)
%     \item HV (Table1-4)
%     \item Inference cost (Table1-4)
%     \item Flexibility (Table1-4)
%     \item Uniformity
%     \item w/o vs w/
%     \item training time
% \end{itemize}
\noindent \textbf{Controllable resource usage.}
We visualize the variation in computational cost with respect to different task and resource usage preferences in Figure~\ref{fig:resource}.
We adopt the ratio of the size of the predicted architecture to the size of the total anchor net as the criterion for evaluating computational cost. 
Compared to conventional dynamic networks that only adjust weights with a fixed computational cost (right), our framework (left) enables control over the total cost via a cost preference $c$. %It is clearly visible that 
Resource usage peaks at the center of the contour, when more tasks are active, and falls down gradually as we move towards the corners, where task preferences are heavily skewed. Furthermore, the average resource usage decreases as $c$ is increased, indicating the ability of the controller to incorporate resource constraints.

\noindent \textbf{Multi-task performance.}
We demonstrate the overall multi-task performance in Tables~\ref{tab:pascal5_perf}-\ref{tab:cifar_perf} on four different %multi-task 
settings (PASCAL-Context 5-task, PASCAL-Context 3-task, NYU-v2 3-task, CIFAR-100 20-task). In all cases, we report hypervolume (reference point mentioned below heading) and uniformity averaged across $20$ task preference vectors $\bm{r}$, sampled uniformly from $\mathcal{S}_N$. Inference network cost is calculated similarly
% in a similar fashion 
over $1000$ preference vectors. These are shown for two choices of $c\in \{0,1\}$ to highlight the two extreme cases of resource usage. 

Our framework achieves higher values in both hypervolume and uniformity compared to the existing dynamic models (PHN and PHN-BN) in all four settings.
While the high hypervolume reinforces the efficacy of tree-structured models in solving multi-task problems, the uniformity values consolidate architectural change as an effective approach towards modeling task trade-offs.
This is accompanied by increased average computational cost, indicated by inference parameter count.
As discussed above, this is due to the flexible architecture over preferences, where actual cost will differ for each preference, \eg, reaching the cost of PHN-BN for extremely skewed preferences (Figure~\ref{fig:resource}). %For uniform preferences, 
Compared to Single-Task, the proposed controller is able to find effective architectures (as indicated by the hypervolume) which perform nearly at par %with the baseline 
with a smaller memory footprint (as indicated by the average inference network parameter count). Notably, in the NYU-v2 3-task and CIFAR-100 settings,
% dynamic architectures are able to 
the ability to find effective architectures enables the model to
outperform single-task networks, demonstrating the benefit of sharing features among related tasks via architectural change.
In addition, our framework enjoys flexibility between two extreme cases, \ie Single-Task (highest accuracy with lowest inference efficiency) and dynamic models with shared backbone (lowest accuracy with highest inference efficiency), spanning a range of trade-offs for different $c$ values. The range of HV is larger when task-specific features are useful, compared to when the compact architecture already achieves higher HV than the Single-Task (Tables~\ref{tab:nyu_perf},\ref{tab:cifar_perf}).
``Control Params.'' is the cost of the hypernets. Note that this overhead will materialize only when the preference changes and does not have any effect on the task inference time.



\input{tables/pascal_5task_1}
\input{tables/pascal_3task_1}
\input{tables/nyu_3task_1}
\input{tables/cifar_20task_1}

\noindent \textbf{Effect of cross-task adaptation}
In Tables~\ref{tab:pascal5_perf}-\ref{tab:cifar_perf}, 
``Ours w/o adaptation'' denotes the model without weight hypernet. As indicated by larger HVs, cross-task adaptation improves the performance without affecting the inference time.
%
A trend that persists across all the settings is the slight drop in uniformity that accompanies the adapted models in comparison to the unadapted ones. This is due to the propensity of the weight hypernet to improve task performance as much as possible while keeping the preferences intact. This leads to improved performance even in the low-priority tasks at the expense of lower uniformity. Note that our primary factor of controllability is through architectural changes which remains unaffected by the weight hypernet.

\noindent \textbf{Training efficiency.}
In contrast to dynamic networks, static multi-task networks require multiple models to be trained, corresponding to different task preferences, to approximate the trade-off curve. As a result, these methods have a clear trade-off between their performance and their training time. To analyze this trade-off, we plot hypervolume vs. training time for our framework when compared to training multiple static models in Figure \ref{fig:multitask_hv}. We trained 20 multi-task models with different preferences sampled uniformly, and at the inference time we selected subsets of various sizes and computed their hypervolume. The shaded area in Figure~\ref{fig:multitask_hv} reflects the variance over different selections of task preference subsets.
%While our framework achieves a $\mathcal{O}(1)$ training time with respect to the number of preferences, these multi-task networks incur a $\mathcal{O}(n)$ training time complexity. \YM{bit risky argument?}
This empirically shows that our approach requires shorter training time to achieve similar hypervolume compared to the static multi-task networks.
% \YM{we may rather want to emphasize the scalability of our method, as 60 hours of training time may not look a significant drawback} \sam{Yup, you could also talk in relative terms, i.e., for 20 preferences training time is 20x (well, probably a bit less b/c of anchornet, hypernet, etc. But in Fig 7, we could also make the x axis relative to the proposed method.}
\input{plots/hv_multitask}

\subsection{Analysis}

\noindent \textbf{Architecture evaluation.}
We study the effectiveness of the architectures predicted by the edge hypernet by comparing them with those predicted by LTB~\cite{guo2020learning} and BMTAS~\cite{bruggemann2020automated}. We choose the architecture predicted for a uniform task preference and, similar to LTB, we retrain it for a fair comparison. We evaluate the performance in terms of relative drop in performance across tasks and number of parameters with respect to the single task baseline. Despite not being directly trained for NAS, our framework is able to output architectures which perform at par with LTB (Table~\ref{tab:nyu_arch}). More results on the Pascal-Context dataset and visualization of dynamic architectures can be found in the supplementary document.

\input{tables/pascal_3task_2}
\input{plots/nyu/nyu_marginals_pgfplot_onecolumn}

\noindent \textbf{Task controllability.}
In Figure \ref{fig:marginal_nyu} we visualize the task controllability for our framework by plotting the test loss at different values of task preference for that specific task, marginalized over preference values of the other tasks. As expected, increasing the preference for a task gradually leads to a decrease in the loss value. Furthermore, increasing $c$ leads to higher loss values due to smaller predicted architectures. The effect of the weight hypernet is also evident, as shown by the lower loss values obtained on using it on top of the edge hypernet (w/o adaptation).
% This is also summarized as uniformity in Table~\ref{tab:pascal5_perf}-\ref{tab:cifar_perf}. %, consolidating architectural change as an effective approach towards modeling task trade-offs.


% \amit{Isn't drop in uniformity problematic? If so, I do not understand the above explanation discounting it.}
% \begin{figure}[t]
% \centering
% \includegraphics[width=.33\columnwidth]{plots/pascal3/pareto/pascal_parts_sal.pdf}\hfill
% \includegraphics[width=.33\columnwidth]{plots/pascal3/pareto/pascal_semseg_parts.pdf}\hfill
% \includegraphics[width=.33\columnwidth]{plots/pascal3/pareto/pascal_semseg_sal.pdf}
% \caption{\textbf{Pareto}}
% \label{fig:nyu_pareto}

% \input{plots/nyu/nyu_marginals_pgfplot_onecolumn}
% \input{plots/pascal3/pascal3_marginals_pgf_onecolumn}

\subsection{Ablation Study} \label{sec:ablation}
\noindent \textbf{Impact of inactive loss.}
Removing $\mathcal{L}_{\textrm{inact}}$ leads to loss of controllability with the edge hypernet predominantly predicting the full original anchor net, with minimal branching, leading to high resource usage and poor uniformity (Table~\ref{tab:nyu_ablation}).

\noindent \textbf{Impact of weighting factors.} 
Removing the two branching weights, $\frac{L-l}{L}$ and $A$, in the active loss, we make three key observations in Table~\ref{tab:nyu_ablation}: 1) average resource usage increases, 2) uniformity drops due to poor alignment between architectures and preferences, with larger architectures incorrectly predicted for skewed preferences, which ideally require less resources, 3) hypervolume remains almost constant across different $c$ indicating poor cost control. Resource usage plots are presented in the supplementary.

\noindent \textbf{Analysis of task threshold.} 
We compare the effect of varying the threshold $\tau$ in Figure~\ref{fig:thresh}. Increasing the value beyond $1/N$ ($\sim 0.3$) leads to loss of controllability as indicated by the constant hypervolume across different values of $c$. This is due to the inability to account for uniform preferences. On the other hand, choosing values below this threshold leads to comparable performance. Additional explanations are provided in the supplementary. 

\noindent \textbf{Task classification.}
We analyse the importance of the induced task dichotomy by considering all tasks as active. This leads to: 1) high overall resource usage, and 2) poor controllability, especially at low values of $c$, as shown in Table~\ref{tab:nyu_ablation}. Resource usage plots are presented in the supplementary.
\input{tables/nyu_ablation}
\input{plots/thresh}


% - describe results \\
% - explain why uniformity decreases for weight hypernet \\
% - highlight outperforming single task on NYUD \\
% - add plots for multi-task baseline
% \vskip 4pt
% \noindent \textbf{Resource Usage Analysis.}
% - describe resource plots
% \vskip 4pt
% \noindent \textbf{Architecture Evaluation.}
% - describe tables for architecture eval \\
% - highlight controllable aspect compared to LTB

% \subsection{Ablation Study}
% \noindent \textbf{Ablation on Training Losses.}
% \vskip 4pt
% \noindent \textbf{Effect of Weighting Factors.}
% \vskip 4pt
% \noindent \textbf{Effect of Threshold.}


% \input{tables/nyu_3task_2}




%\begin{figure*}
%\centering
%\begin{subfigure}[b]{0.32\textwidth}
%\includegraphics[width=\linewidth]{plots/nyu/nyu_semseg.pdf}
%\caption{Semantic Segmentation}
%\label{fig:nyu_marginal_semseg}
%\end{subfigure}
%\begin{subfigure}[b]{0.32\textwidth}
%\includegraphics[width=\linewidth]{plots/nyu/nyu_normals.pdf}
%\caption{Surface Normals}
%\label{fig:nyu_marginal_normals}
%\end{subfigure}
%\begin{subfigure}[b]{0.32\textwidth}
%\includegraphics[width=\linewidth]{plots/nyu/nyu_depth.pdf}
%\caption{Depth}
%\label{fig:nyu_marginal_depth}
%\end{subfigure}
%\caption{\textbf{Marginal evaluation on NYUD-v2}}
%\label{fig:marginal_nyu}
%\end{figure*}


%\begin{figure*}
%\centering
%\begin{subfigure}[b]{0.32\textwidth}
%\includegraphics[width=\linewidth]{plots/pascal3/pascal3_semseg.pdf}
%\caption{Semantic Segmentation}
%\label{fig:pascal3_marginal_semseg}
%\end{subfigure}
%\begin{subfigure}[b]{0.32\textwidth}
%\includegraphics[width=\linewidth]{plots/pascal3/pascal3_parts.pdf}
%\caption{Surface Normals}
%\label{fig:pascal3_marginal_parts}
%\end{subfigure}
%\begin{subfigure}[b]{0.32\textwidth}
%\includegraphics[width=\linewidth]{plots/pascal3/pascal3_sal.pdf}
%\caption{Depth}
%\label{fig:pascal3_marginal_sal}
%\end{subfigure}
%\caption{\textbf{Marginal evaluation on PASCAL-Context (3 tasks)}}
%\label{fig:marginal_pascal3}
%\end{figure*}


%\begin{figure}
%\centering
%\includegraphics[width=0.9\columnwidth]{plots/thresh.pdf}
%\caption{\textbf{Varying thresholds on NYUD-v2}}
%\label{fig:thresh}
%\end{figure}


% \paragraph{Datasets} \mbox{}\\
% 1. Pascal~\cite{mottaghi2014the}\\
% 2. NYU~\cite{silberman2012indoor}\\
% % 3. Rich Human\\
% 3. Tiny Taskonomy~\cite{zamir2018taskonomy}? (\ym{Scalability})

% \paragraph{Evaluation criterion} \mbox{}\\
% 1. Accuracy: Pareto curve, HyperVolume\\
% 2. Controllability: Uniformity, Marginal accuracy profile, Relative loss profile\\
% 3. Computational cost: FLOPs of the feature extractor and hypernets\\
% 4. Training time\\
% 5. Dynamic range (with cost?)\\
% 6. Memory


% \paragraph{Comparison} \mbox{}\\
% Upper bound:
% single-task networks\\
% Baselines:
% multi-head network\\
% + EPO?~\cite{}
% PHN~\cite{navon2021learning}\\
% Ctrl Pareto MTL~\cite{lin2020controllable}\\
% LTB~\cite{guo2020learning}\\
% BMTAS~\cite{bruggemann2020automated}\\
% PMTL, PCMTL? \\

% \subsection{Evaluation and Analysis}
% \YM{test for larger models?}
% \begin{itemize}
%     \item Comparison with baselines\\
%     Method: Ours, baselines, upper bound. \\
%     Measure: HV, uniformity, computational cost, training time\\
%     Tables/figures: One table for each dataset
    
%     \item Comparison with baselines\\
%     Method: Ours, baselines, upper bound. \\
%     Measure: Pareto curve, marginal accuracy profile, relative loss profile\\
%     Tables/figures: One figure for each dataset
    
%     \item Edge-hypernet performance\\
%     Method: Ours w/o weight-hypernet + re-training, BMTAS, LTB \\
%     Measure: Task performance \\
%     Tables/figures: 
    
%     \item Ablation study (losses)\\
%     Method: Ours - w/o active loss, w/o inactive loss   \\
%     Measure (w/o inactive loss): loss of control (HV same, lower uniformity) \\
%     Measure: (w/o active loss): more resource utilization (HV same, slightly lower uniformity, constantly more resource utilization)
%     Tables/figures: 1 Table for HV/Uniformity, 1 figure for cost difference
    
%     \item cost control
    
%     \item Robustness to hyper parameter choice
%     \item Generalization to unseen preferences
%     \item Architecture visualization?
% \end{itemize}

% \begin{table}[t]
% 	\caption{
% 	Comparison on the NYUv2 dataset
% 	}\label{table:nyuv2}
% % 	\small
% 	\begin{center}
% 	\setlength{\tabcolsep}{2pt}
% 	\begin{tabular}{lcccc}
% 		\toprule
% 		Method & HV & Uniformity & FLOPs & Training time \\
% 	    \midrule
% 	    Single-task networks & &  &\\
% 	    \midrule
%         Multi-head network (LS) &  & & \\
%         EPO &  & & \\
%         % PMTL &  & & \\
%         % PCMTL &  & & \\
%     	\midrule
%         PHN-LS~\cite{navon2021learning} & & & \\
%         PHN-EPO~\cite{navon2021learning} & & & \\
%         Ctrl Pareto MTL~\cite{lin2020controllable} & & & \\
%         \midrule
%         Ours & & & \\
% 		\bottomrule
% 	\end{tabular}
% 		\end{center}
% % \vspace{-5mm}
% \end{table}


==> sections/method.tex <==
\section{Method}

Given a set of $N$ tasks $\mathbf{T}=\{\mathcal{T}_1,\mathcal{T}_2,\dots,\mathcal{T}_N\}$, conventional \emph{static} multi-task learning seeks to minimize a weighted sum of task-specific losses: $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$, where each $\mathcal{L}^i$ represents the loss associated with task $\mathcal{T}_i$, and $\bm{r} \in \mathcal{S}_N$, where $\mathcal{S}_N=\{\bm{r}\in\mathbb{R}^N | \sum_i r_i = 1, r_i \geq 0\}$ represents the $N$-dimensional simplex~\cite{ruder2017overview}. Here, $\bm{r}$ denotes a task preference vector signifying the desired trade-off over the different tasks, where larger values of $r_i$ attribute higher importance to task $\mathcal{T}_i$. Typically, one needs to re-train the model from scratch every time the desired task preferences change. 

To overcome re-training from scratch , recent approaches~\cite{navon2021learning,lin2020controllable} propose to learn the entire trade-off curve for the multi-task problem by predicting model weights conditioned on $\bm{r}$. 

In contrast, we propose a framework which goes beyond a fixed model architecture and approximates this trade-off curve in terms of \emph{model structure}. We design a controller based on \textit{hypernetworks}~\cite{ha2016hypernetworks}, which takes as input a task preference $\bm{r}$ to dynamically allocate model resources among the tasks in proportion to the supplied preference. Beyond the task preferences, we also add provisions for control over total resource usage using an additional resource preference variable $c \in [0,1]$, where increasing values of $c$ forces the controller to be more frugal while allocating resources. Crucially, the choice of varying architecture as a means to model the task trade-offs allows us to dynamically control resource allocation within a single multi-task model.\YM{I am not sure what was intended with the last sentence. Isn't the conventional weight-only dynamic hypernet also allows dynamic control for resource allocation among tasks?}
\ym{Crucially, the choice of varying architecture as a means to model the task trade-offs allows a larger variation within a single multi-task model. This leads to ..?}

To allow for such dynamic architectural changes we first define a network search space in Section \ref{sec:search_space}. This is followed by a description of the proposed two-stage training strategy: first, a preference agnostic supernet is trained to enforce task priors, as outlined in Section \ref{sec:supernet}; the trained supernet is subsequently used in the second stage of training by the hypernetworks, which are described in Section \ref{sec:hypernet}. \ym{Overview of our method is illustrated in Figure~\ref{fig:overview}.}

\subsection{Network Search Space} \label{sec:search_space}
Dynamic architectural changes require a search space which can represent a wide variety of architectures. In this work, we utilize a tree-structured network topology which has been shown to be highly effective for multi-task learning in \cite{guo2020learning, bruggemann2020automated}.
Since tree-structured networks share common low-level features over tasks while extracting task-specific ones in the higher layers, we expect to control the trade-off by learning to change the branching locations conditioned on the joint preference $\left(\bm{r},c\right)$.

The search space is represented as a \textit{directed acyclic graph } (DAG), where vertices in the graph represent numerical operations (convolution, pooling etc.) and edges denote the data flow through the network. Figure \ref{fig:block} shows a block of such a graph, containing $N$ \textit{parent} and \textit{child} nodes. The tree-structure is realized by stacking such blocks sequentially and allowing a child node to sample a path from the candidate paths between itself and all its parent nodes. Concretely, the branching operation at layer $l$ can be formulated as:
% \YM{expectation necessary in the equation?}
% \begin{equation} \label{eq:branching}
%     x^{l+1}_j = \mathbb{E}_{d_j\sim p_{\alpha_j^l}} \left[d_j\cdot Y^l\right],
% \end{equation}
\ym{
\begin{equation} \label{eq:branching}
    x^{l+1}_j = \sum_{j} d_j\cdot y^l_j,
\end{equation}
}
where $x^{l+1}_j$ denotes the input to the $j$-th node in layer $l+1$, $d_j$ is a one-hot vector indicating the parent node sampled from the \emph{categorical} branching distribution parameterized by $\alpha_j^l$ and, \ym{$y^l_i$ is the output of $i^{th}$ node at layer $l$.} %$Y^l = [ y^l_1, \dots, y^l_N ]$ concatenates outputs from all parent nodes at layer $l$. 
The set of distribution parameters $\bm{\alpha} = \{\alpha_j^l\}_{j \leq N, l < L}$ control the overall structure of the network. This dependence suggests learning these parameters, conditioned on a preference $(\bm{r},c)$, in a manner which satisfies the desired performance trade-off. We describe this learning process in the following sections.
\YM{fix equation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{images/branching_block.pdf}
    \caption{\textbf{Branching block.} Illustration of the parent sampling operation from Eqn. \ref{eq:branching}. Nodes in layer $l$ are sampled in accordance to a categorical distribution defined by $\alpha^l_j$ $\left(\sum_i \alpha^l_j(i)=1\right)$ for each node $(l+1,j)$ in layer $l+1$.}
    \label{fig:block}
    \vskip -12pt
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/framework.pdf}
    \caption{\textbf{Framework}\XY{add illustration}}
    \label{fig:framework}
\end{figure*}

\subsection{Initialization via Weight-Sharing} \label{sec:supernet}
% \YM{Conventional strategy for neural architecture search is to formulate the problem as a bi-level optimization. It seeks optimal network architecture that minimizes objective computed from optimal weights found in the first-level optimization given the architecture~\cite{}}.

The conventional strategy for neural architecture search methods is to formulate the search as a bi-level optimization problem~\cite{liu2018darts}, where model weights and architecture are optimized alternately with respect to a fixed training loss.
% \begin{equation}
% \begin{split}
%     & \min_{\bm{\alpha}} \ \mathcal{L}\left(w^*(\bm{\alpha}), \bm{\alpha}\right) \\ 
%     & \text{s.t.} \ w^*(\bm{\alpha}) = \min_{w} \ \mathcal{L}\left(w,\bm{\alpha}\right)
% \end{split}
% \end{equation}
% \YM{formulation for our problem?}
% where $w$ represents the model weights, $\bm{\alpha}$ determines the network architecture and $\mathcal{L}$ denotes the training loss. 
In our case, the presence of a preference tuple $(\bm{r},c)$ in the loss function implies solving this expensive optimization procedure for \emph{every} possible preference - this makes the entire process infeasible.

% \YM{as this is to motivate 2-stage training, add explanation of hypernet to explain how $\bm{r}$ adds additional layer of complexity?}
% \YM{
% \begin{align}
% \min_{\phi, \psi} \mathbb{E}_{\mathbf{r}}[L_{\mathbf{r}}(\alpha, w)] \\
% \text{where } \alpha = \Phi(\mathbf{r}, \phi), w = \Psi(\mathbf{r}, \psi)
% \end{align}
% }

In order to simplify the problem, we take inspiration from one-shot neural architecture search methods which advocate sharing weights between models by training a \textit{supernet}: rather than training thousands of separate models from scratch, one can train a single large network capable of emulating any architecture in the search space \cite{bender2018understanding}. Once the supernet has been trained, architectures can be directly evaluated for their suitability for any preference $(\bm{r},c)$ by inheriting the fixed weights from the supernet, instead of re-training each time an architecture is chosen for a given preference.

% \YM{Concept of supernet contains every potential edge, so I guess better to avoid specifying alpha as a fixed (fully-branched) structure. We only need to describe the supernet weight initialization. How about omitting exact equations if text can deliver the meaning clearly?}
\iffalse
With the downstream task of dynamic architectural changes in consideration, we propose to compose the supernet $F$ as a collection of single-task networks. In terms of the parent-child blocks defined in the previous section, the branching distribution parameters are defined as:
\begin{equation}
    \alpha_j^l = \mathbf{e}_j, \ \forall \  j \in [N], \  l \in [L],  
\end{equation}
where $\mathbf{e}_j$ denotes the $j$-th standard basis vector of $\mathbb{R}^N$ (see Figure \ref{fig:supernet}). Thus, node $j$ in any layer corresponds to the the task $t_j$.
% \YM{in the previous definition, $\alpha$ parameterize $P_{\alpha}$ but function is not defined yet}
Using this fully branched structure, the supernet weights are trained to minimize the following loss:
\begin{equation}
    \mathcal{L}_{sup} = \sum_{i=1}^N\mathcal{L}^i.
\end{equation}
At the conclusion of training, we obtain the optimal weights $w^*$ of the supernet $F$. Note that the training of the supernet is completely preference agnostic, and serves solely to provide a prior for the subsequent stage. 
\fi
With the downstream task of dynamic architectural changes in consideration, we propose to initialize the supernet with weights $w^*$, equivalent to a collection of single-task networks as illustrated in Fig.~\ref{fig:framework}(a). This allows sufficient differentiation among individual task streams with distinct features, which was empirically crucial to induce architectural changes in the subsequent stages. While the supernet trained in such a manner does not capture cross-task edges, it is very effective as: (i) it allows for designing task relationships based on observations in \cite{vandenhende2019branched}, where branching in tree-structured multi-task networks is contingent on how similar task features are at any layer, and (ii) can be further enriched to reflect cross-task edges by the proposed controller via modulation of normalization parameters.

% This choice serves as an effective prior since it allows for designing task relationships based on observations in \cite{vandenhende2019branched}, where branching in tree-structured multi-task networks is contingent on how similar task features are at any layer. Furthermore, this allows sufficient differentiation among streams with specified features for individual tasks, which was empirically crucial to induce architectural changes to be learned in the subsequent stages. 

% Our choice of initializing the supernet with single-task networks stems from observations in \cite{vandenhende2019branched}, where branching in tree-structured multi-task networks is contingent on how similar task features are at any layer. Thus, a supernet trained in such a manner provides sufficient information for learning the branching distribution parameters.
% \ym{This allows sufficient differentiation among streams with specified features for individual tasks, which was empirically crucial to induce architectural changes to be learned in the second stage.}
% \YM{Added to reflect Samuel's comment that empirical justification of fully-branched initialization could be added, as in some sense this looks contradicting to weight-sharing philosophy}

\subsection{Preference Conditioned Hypernetworks} \label{sec:hypernet}
\YM{Loss formulation is sufficiently explained, but input formulation (tokens) and network architectures are missing. arch details could be added to implementation details}
As described in Section \ref{sec:search_space}, every possible architecture in consideration is described concisely by the set of branching parameters $\bm{\alpha}$. Since the number of potential configurations grows exponentially with the number of layers and tasks, it becomes intractable to manually find the optimal architecture for every possible preference vector.
% \YM{complexity grows exponentially with the number of tasks?}
Thus, we propose to train a hypernetwork \cite{ha2016hypernetworks} based controller to sample optimal tree-structured architectures from the trained supernet to satisfy the given preferences. \footnote{Note that when we mention that the controller samples architectures, we wish to convey that it predicts the parameters of the branching distributions from which we sample the tree structures. We follow this for conciseness.}

Concretely, we train a hypernetwork $h$, parameterized by $\phi$, to predict the branching parameters $\hat{\bm{\alpha}}=h(\bm{r},c; \phi)$ within the supernet $F$. Since we wish to control the resource allocation at the inference time, the hypernetwork should learn to perform architectural changes for a \emph{distribution} $P_{(\bm{r},c)}$ of valid preference vectors rather than a single one. Hence, during training time the model observes many losses, defined by preferences $\bm{r},c\sim P_{(\bm{r},c)}$, and can learn to utilize the relationships between them to optimize all of them simultaneously. At test time, when a preference $(\bm{r},c)$ is presented to the hypernetwork, the optimal tree-structure corresponding to the supplied task and resource preference is sampled from the branching distribution parameterized by the predictions of $h$, and is used directly for inference in $F$. 

\subsubsection{Branching regularized linear scalarization}
To ensure alignment between the preference and the architecture predicted by the hypernetwork, we propose a branching regularized loss function to train the hypernetwork:
\begin{equation}
    \mathcal{L}_{tot}(\bm{r}) = \mathcal{L}(\bm{r}) + \Omega(\bm{r},c).
\end{equation}
As described previously, $\mathcal{L}(\bm{r})$ denotes the \emph{linear scalarization} of the task specific losses, with the task preference vector $\bm{r}$ as loss weights, i.e. $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$. Optimizing this weighted sum only takes into account the individual task performances without explicitly focusing on the resource allocation within the supernet. In order to control resource allocation, we require a node sharing mechanism which complies with the resource preference $c$ by incorporating the task affinities which implicitly exist in the multi-task learning setup. Consequently, we introduce a branching regularizer $\Omega(\bm{r},c)$ to encourage such node sharing (or branching) based on the preference.
\vskip 4pt
\noindent \textbf{Task dichotomy.} The core hypothesis that underlies the choice of the branching regularizer is that \emph{not all tasks influence the branching structure equally}. Consequently, we design this regularizer such that given a preference vector $\bm{r}$, low preference tasks are neglected in favor of the high preference ones in order to save computation and meet resource constraints. To make this distinction concrete, we first define a threshold $\gamma$ and then categorise the tasks into \emph{active} tasks $\mathcal{A}=\{t_i \ | \ r_i \geq \gamma, \ \forall i \in [N]\}$, and \emph{inactive} tasks $\mathcal{I}=\{t_i \ | \ r_i < \gamma, \ \forall i \in [N]\}$. Based on this classification of tasks, we define two losses, each pertaining to one of the groups, which jointly constitute the regularizer $\Omega(\bm{r},c)$. 
\vskip 4pt
\noindent \textbf{Active loss.} We introduce a loss function $\mathcal{L}_{active}$ that encourages nodes in the supernet, corresponding to the active tasks, to be shared in order to avoid the whole network being split up by tasks with little knowledge shared among them. The overall loss is additionally weighted by the resource preference $c$ to control the total resource sharing. \YM{move c to Eq.(12)?} Specifically, we minimize the weighted sum of pairwise $L_2$ distances between the sampled parent edges of the nodes pertaining to the active tasks. Formally, we define $\mathcal{L}_{active}$ as,
\begin{equation} \label{eq:active}
    \mathcal{L}_{active} = c\cdot\sum_{l=1}^L \sum_{\substack{i,j \in \mathcal{A} \\ i\neq j}}
    W(l,i,j)\cdot
    \|\nu^{l}_{i} - \nu^{l}_{j}\|^2,
\end{equation}
\ym{
\begin{equation} \label{eq:active}
    \mathcal{L}_{active} = c\cdot\sum_{l=1}^L \sum_{\substack{i,j \\ i\neq j}}
    W(l,i,j)\cdot
    \|\nu^{l}_{i} - \nu^{l}_{j}\|^2,
\end{equation}
}
% \begin{equation} \label{eq:active}
%     \mathcal{L}_{active} = c\cdot
%     \sum_{l=1}^L \sum_{\substack{i,j}}
%     \mathbb{E} [
%     W_{dep}(l) \cdot T_{rel}(i,j)
%     \cdot
%     \|\nu^{l}_{i} - \nu^{l}_{j}\|^2
%     ],
% \end{equation}
\YM{sum over all i,j? i,j under $\sum$ are task indices and i,j in $\nu_i$, $\nu_j$ are node indices. They may not always match}
where we use the Gumbel-Softmax reparameterization trick \cite{jang2016categorical} to obtain the samples $\nu^l_i$ from the predicted logits $\hat{\bm{\alpha}}$,
\begin{equation} \label{eq:gumbel}
    \nu^{l}_{i}(k) = \frac{\exp \left((\log \alpha^l_i(k) + G^l_i(k))/\tau\right)}{\sum_{m=1}^N\exp \left((\log \alpha^l_i(m) + G^l_i(m))/\tau\right)}.
\end{equation}
Here, $G^l_i=-\log (-\log U^l_i)$ is a standard Gumbel distribution with $U^l_i$ sampled from a uniform i.i.d. distribution $\text{Unif}(0, 1)$. 

The weight $W(l,i,j)$ in Eqn. \ref{eq:active} reflects how much we want any pair of active tasks to share nodes. We factorize this weight into four components: 
\begin{equation}
    W(l,i,j) = P_{use}(l,i) \cdot P_{use}(l,j) \cdot W_{dep}(l) \cdot T_{rel}(i,j) .
\end{equation}

% \YM{Can we add another figure that shows $\alpha$s in the layers to help interpreting notations?}

The factor $P_{use}(l,i)$ represents the probability that the node $i$ at layer $l$ is present in the tree structure that is sampled by the hypernetwork. This factor ensures that the loss is applied correctly to only the nodes which are a part of the sampled architecture. We follow a dynamic programming approach to calculate this value. Denoting the $i^{th}$ node in the $l^{th}$ layer as $(l,i)$, we can define the marginal probability that the node $(l+1,k)$ samples the node $(l,i)$ as its parent as $\nu^{l}_k(i)$.  Thus, the probability that the node $(l,i)$ is used in the sampled tree structure is
\ym{
\begin{equation}
    P_{use}(l,i)
    = 1 - \prod_{k}\{ 1 - P_{use}(l+1,k) \cdot \nu^{l}_k(i) \},
    % = 1 - \prod_{k}\{ 1 - P_{use}(l+1,k)P_{par}(l, i \rightarrow k) \},
    % = \sum_{j} { P_{par}(l, i \rightarrow j) P_{use}(l+1, j)},
\end{equation}
where $P_{use}(L,i) = 1$ for all $i \in [N]$.}
% where,
% \begin{align}
%     P_{use}(L-1,i)
%     &= 1 - \prod_{k} \left(1 - P_{par}(L-1, i \rightarrow k)\right) \nonumber \\
%     &= 1 - \prod_{k} \left(1 - \nu^{L-1}_k(i)\right).
% \end{align}

The factor $W_{dep}(l)$ encourages more sharing of nodes which contain low-level features. This is based on the fact that deep networks share low-level features over tasks while extracting task-specific ones in the higher layers, 
\begin{equation}
    W_{dep}(l) = \frac{L-l}{L}
\end{equation}

The final factor $T_{rel}(i,j)$ captures the \emph{task affinity} or task relatedness between tasks $\mathcal{T}_i$ and $\mathcal{T}_j$. If two tasks are unrelated, sharing of features can lead to degradation of performance, a phenomenon termed as \emph{negative transfer} \cite{liu2019loss}. To this end, we base the layer sharing on measurable levels of task affinity: two tasks are strongly related, if their single task models rely on a similar set of features. We adopt \emph{Representational Similarity Analysis} (RSA) \cite{dwivedi2019representation} to obtain the task affinity scores from the supernet $F$.
\YM{move details of affinity calculation to supple?}
First, using a subset of $K$ instances, we extract the features for each of these data points for every task. Let us denote the extracted feature for instance $k$ at layer $l$ for task $t_i$ as $\bm{f}_{[i,l,k]}$. Using these features, we compute the feature dissimilarity tensor $\mathbf{D}_l$ at each layer, of dimensions $N\times K \times K$, as follows,
\begin{equation}
    \mathbf{D}_l \left(i,j,k\right) = 1 - \frac{\langle\bm{f}_{[i,l,j]},\bm{f}_{[i,l,k]}\rangle}{\|\bm{f}_{[i,l,j]}\|\|\bm{f}_{[i,l,k]}\|}.
\end{equation}
The task affinity matrix $\bm{T}_l$ at layer $l$, of dimensions $N \times N$, is calculated as follows,
\begin{equation}
    \bm{T}_l(i,j) = \|\mathbf{D}_l \left(i,:,:\right)-\mathbf{D}_l \left(j,:,:\right)\|_{F}.
\end{equation}
The factor $T_{rel}(i,j)$ is obtained by taking the mean of the affinity scores across layers, i.e., $T_{rel}(i,j)=\frac{1}{L}\sum_l\bm{T}_l(i,j)$.
\vskip 4pt
\noindent \textbf{Inactive loss.} 
The inactive tasks should have minimal effect in terms of branching. To encourage this behavior, we introduce $\mathcal{L}_{inactive}$ to encourage these tasks to mimic the most closely related branching pattern, 
\begin{equation}
    \mathcal{L}_{inactive} = \sum_{l} \sum_{j \in \mathcal{I}}
     \min_{i \in \mathcal{A}} \|\nu^{l}_{i} - \nu^{l}_{j}\|^2.
\end{equation}
This ensures that the network branching is controlled by the active tasks, with the inactive tasks sharing nodes with the active tasks.

Thus, the branching regularizer is defined as follows,
\begin{equation}
    \Omega(\bm{r},c) = \lambda_{\mathcal{A}}\mathcal{L}_{active} + \lambda_{\mathcal{I}}\mathcal{L}_{inactive},
\end{equation}
where $\lambda_{\mathcal{A}}$, $\lambda_{\mathcal{I}}$ are hyperparameters to determine the weighting of the losses. \XY{simply attach some empirical/typical value  for the weighting here}

\subsubsection{Hypernetwork for cross-task adaptation}
The architecture sampled by the hypernetwork $h$ contains edges which have not been observed during the supernet training. We denote these as \emph{cross-task} edges in relation to the fact that these edges connect nodes belonging to different tasks in the supernet. Consequently, the performance of the sampled network is sub-optimal. To rectify this issue, we need to fine-tune the weights of $F$ to adapt it these unseen edges. In order to preserve the online nature of our framework we use an additional hypernetwork $\bar{h}$ to predict the fine-tuned weights of the architecture sampled by $h$. 

However, $F$ is non-linear and its parameters can be high dimensional, making optimization too sensitive and inefficient for online prediction. As an alternative to fine-tuning all the model’s parameters, prior work \cite{wang2020tent} estimates normalization statistics and optimizes channel-wise affine transformations. Following suit, we propose to generate normalization parameters using a hypernetwork in order to capture the cross-task information to enhance the final performance.

Conventional batch normalization at layer $l$ for node $i$ is defined as,
\begin{align}
    \text{BN}_i^l(\bm{x}^l_i) = \gamma^l_i\frac{x^l_i-\mu^l_{i}}{\sigma_i^l} + \beta^l_i,
\end{align}
where $\gamma^l_i$ and $\beta^l_i$ are the learnable parameters, and $\mu^l_i$ and $\sigma^l_i$ denote the batch statistics of the node input $x^l_i$. Given a preference $(r,c)$ and predicted branching parameters $\hat{\bm{\alpha}}=h(\bm{r},c; \phi)$, we predict perturbations to the batch normalization parameters using $\bar{h}$: $\{\Delta \gamma^l_i,\Delta \beta^l_i\}_{i \leq N, l < L} = \bar{h}(r,c;\theta)$. This allows us to redefine the batch normalization layers as follows, 
\begin{align}
    \text{BN}_i^l(\bm{x}^l_i) = (\gamma^l_i+\Delta\gamma^l_i)\frac{x^l_i-\mu^l_{i}}{\sigma_i^l} + (\beta^l_i+\Delta\beta^l_i).
\end{align}

We train $\bar{h}$ by first sampling preferences $\bm{r},c\sim P_{(\bm{r},c)}$ and the architecture from the hypernetwork $h$ trained previously, and then apply the predicted normalization parameter perturbations along the sampled architecture to optimize the linear scalarized task losses $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$.

% % - weighted loss and branching \\
% % - active/inactive tasks \\
% % - active loss \\
% % - inactive loss \\
% % - task similarity computation






% % \paragraph{Hypernetwork for edge prediction} \mbox{}\\
% % - task similarity matrix computation \\
% % - linear scalarization \\
% % - branching losses 
% % \paragraph{Hypernetwork for cross-connections adaptation}

% % \paragraph{Algorithm} \mbox{}\\






% % Consider a supernet that consists of $T$ streams for $T$ tasks.
% % Each stream consists of $L$ sequential modules where $L^{th}$ layer corresponds to the task-specific head.
% % Let us denote the $i^{th}$ node in the $l^{th}$ layer as $(l,i)$.
% % % To simplify notation, we denote the input image as the node of the $0^{th}$ layer.
% % At each trial, each node independently samples its parent node.
% % Once every node selects its parent, the network architecture is specified to the corresponding tree structure.
% % Note that different combinations of parent selections can havet the same tree structure.
% % %For example,

% % We define the marginal probability that the node $(l+1,j)$ choose $(l,i)$ as its parent as
% % \begin{equation}
% %     P_{par}(l, i \rightarrow j)
% %     = \frac{\exp(\alpha^{l+1}_{j,i} / \tau)}
% %       {\sum_{k}{\exp(\alpha^{l+1}_{j,k} / \tau)}}.
% % \end{equation}
% % % Here, $\alpha^{l}_{i,j}$ is a scalar.
% % The sample space is the set of all possible combinations of parent selections as shown in Figure~\ref{fig:sample_space}.
% % The probability that the node $(l,i)$ is used in the tree structure is
% % \begin{align}
% %     P_{use}(l,i)
% %     = 1 - &\prod_{j}\{ 1 - P_{use}(l+1,j)P_{par}(l, i \rightarrow j) \}
% %     % = \sum_{j} { P_{par}(l, i \rightarrow j) P_{use}(l+1, j)},
% % \end{align}
% % where
% % \begin{align}
% %     P_{use}(L-1,i)
% %     &= 1 - \prod_{j} (1 - P_{par}(L-1, i \rightarrow j)) \nonumber \\
% %     &= 1 - \prod_{j} (1 - \frac{\exp(\alpha^{L}_{j,i} / \tau)}
% %                               {\sum_{k}{\exp(\alpha^{L}_{j,k} / \tau)}}).
% % \end{align}


% % Active loss is formulated as
% % \begin{equation}
% %     L_{act} = \sum_{l} \sum_{\substack{i,j \\ i\neq j}}
% %     P_{use}(l,i) P_{use}(l,j)
% %     % (\sum_{t \in \mathcal{A}} P_{task}(l,i,t))
% %     % (\sum_{t \in \mathcal{A}} P_{task}(l,j,t))
% %     \|\alpha^{l}_{i,\cdot} - \alpha^{l}_{j,\cdot}\|^2,
% % \end{equation}
% % where
% % % $\mathcal{A}$ is the set of active tasks and 
% % $\alpha^l_{i,\cdot} = [\alpha^l_{i,1}, \cdots, \alpha^l_{i,t}]\in \mathbb{R}^T$.

% % Inactive loss is formulated as
% % {\color{red}
% % \begin{equation}
% %     L_{inact} = \sum_{l} \sum_{j}
% %     (1 - P_{use}(l,j))
% %      \min_{i} P_{use}(l,i) \|\alpha^{l}_{i,\cdot} - \alpha^{l}_{j,\cdot}\|^2,
% % \end{equation}
% % }

% % The expected number of used nodes in the tree structure is
% % \begin{equation}
% %     \sum_{l,i} P_{use}(l,i).
% % \end{equation}

% % \ym{scalability}

==> sections/method_1108.tex <==
% \newpage
\section{Preliminaries}
% tasks
% loss
% r and c
Given a set of $N$ tasks $\mathbf{T}=\{\mathcal{T}_1,\mathcal{T}_2,\dots,\mathcal{T}_N\}$, conventional multi-task learning seeks to minimize a weighted sum of task-specific losses: $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$, where each $\mathcal{L}^i$ represents the loss associated with task $\mathcal{T}_i$, and $\bm{r} \in \mathcal{S}_N$, where $\mathcal{S}_N=\{\bm{r}\in\mathbb{R}^N | \sum_i r_i = 1, r_i \geq 0\}$ represents the $N$-dimensional simplex~\cite{ruder2017overview}. Here, $\bm{r}$ denotes a task preference vector signifying the desired trade-off over the different tasks, with larger values of $r_i$ denoting higher importance to task $\mathcal{T}_i$. 
Our objective is to approximate the trade-off curve defined by different values of $\bm{r}$ using tree-structured sub-networks within a single multi-task model. The search space is further constrained by a resource preference variable $c \in [0,1]$, which takes into account the compute cost of the predicted architectures - increasing values of $c$ forces the controller to be more frugal while allocating resources and vice-versa.
\ym{In this paper, we assume that fast inference is more important while model size is relatively cheap. We believe this assumption matches many practical applications where real-time inference is required.}

% we also add provisions for control over total resource usage using an additional resource preference variable $c \in [0,1]$, where increasing values of $c$ forces the controller to be more frugal while allocating resources.
% Typically, one needs to re-train the model from scratch every time the desired task preferences change.
% \YM{please change this to show connection between r and c.}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{images/branching_block.pdf}
    \caption{\textbf{Branching block.} Illustration of the parent sampling operation in Section \ref{sec:search_space}. Nodes in layer $l$ are sampled in accordance to a categorical distribution defined by $\alpha^l_j$ $\left(\sum_i \alpha^l_j(i)=1\right)$ for each node $(l+1,j)$ in layer $l+1$.}
    \label{fig:block}
    \vskip -12pt
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/framework.pdf}
    \caption{\textbf{Framework}\XY{add illustration}
    \YM{Remove figure of branching regularization. Leave 'branching regularzation and Omega, Eq. Change Omega to contain r,c. Move subfigure to another figure to explain active and inactive loss.}
    }
    \label{fig:framework}
\end{figure*}


\section{Method}
\YM{method section is not done yet}
% \YM{Instead of describing general hypernetwork, let's focus more on describing our own design choices and the underlying reasons -- 1) 'tree-structured' dynamic architecture 2) supernet + edge hypernet + weight hypernet instead of edge hypernet + weight hypernet.
% }
% Goal: train hypernetwork that enables test-time arch & weight generation while controlling accuracy trade-off and compute budget
% Tree structured network generation at test time
Our goal is to train a multi-task model that adjusts its architecture and weights to match the user defined task importance scores and computational budget restrictions at test-time. We cast this problem as a form of dynamic controllable architecture search, where we constrain the architectures to a tree-structured topology, as defined in Section~\ref{sec:search_space}. %This is based on two observations: 1) tree-structured network topology is highly effective for multi-task learning, as shown in \cite{guo2020learning, bruggemann2020automated}, and 2) the search space is highly expressive, giving rise to a wide variety of architectures for different task combinations.
% We constrain the architectures to a tree-structured topology defined in Section~\ref{sec:search_space} based on two observations: 1) tree-structured network topology is highly effective for multi-task learning in \cite{guo2020learning, bruggemann2020automated} and 2) the optimal structure differs for different target task combination.
Using this search space, we aim to design a controller which can flexibly generate tree-structured models at test time.  
% In a nut shell, we aims at flexibly generating a tree-structured model at test time.

% System organization overview & inference
% Challenge in weight generation
% -> Introduce supernet + weight hypernet adjusts only BN affine params 
% (vs. weight hypernet generating full weigths)
% Inference
% Connection to overview figure
To this end, we introduce two \textit{hypernetworks}~\cite{ha2016hypernetworks} that take the user preference $(\bm{r}, c)$ as input and define a tree-structured multi-task network, along with its weights, within the search space.
We denote the first hypernetwork as the \emph{edge hypernet}, and the second one as the \emph{weight hypernet}. While the edge hypernet outputs the architecture, the weight hypernet predicts the weights for the predicted architecture. 
Since it is costly to generate all the network weights, we propose an alternative approach, \ie, we employ an \emph{anchor network} with fixed weights and adapt only a portion of the weights in accordance with the trade-offs. 

The anchor network is composed as a collection of $N$ streams of backbones and serves two key purposes. First, it enables the edge hypernet to search for efficient architectures over the tree-structured topology. This is crucial to make search realizable as most NAS methods formulate the search as a bi-level optimization problem~\cite{liu2018darts}, where model weights and architecture are optimized alternately with respect to a fixed training loss. In our case, the presence of a preference tuple $(\bm{r},c)$ in the loss function implies solving this expensive optimization procedure for \emph{every} possible preference - this makes the conventional process infeasible. Second, the anchor serves as the base weights over which the weight hypernet makes it predictions. Specifically, the weight hypernet predicts the parameters of the normalization layers to adapt the anchor network to the predicted architecture. Such adaptation using modulation of the normalization parameters have been successfully applied in NLP~\cite{mahabadi2021parameter}. At test-time, given an input preference, we take predictions of architectures and weights from two hypernets and combine them with the anchor weights from the supernet to generate the final network, which is used to obtain the actual task predictions for the input image as illustrated in Figure~\ref{fig:framework} (c).


% Specifically, to enable the search over the tree-structured topology, we compose the anchor network as a collection of $N$ streams of backbones. 
% Using it as an anchor, batch normalization affine parameters are only adjusted via the weight hypernet while edges are activated vie edge hypernet.
% At test-time, given an input preference, we take predictions of architectures and weights from two hypernets and combine them with the anchor weights from the supernet to generate the final network, which is used to obtain the actual task predictions for the input image as illustrated in Figure~\ref{fig:framework} (c).
\YM{Add outcomes and concerns from introducing anchornet: more memory. However, this is not an issue based on the explanation from computation resource in 4.Preliminaries}

% Challenge in training: jointly training of arch and weight is difficult
% -> 3-stage training: 
% 1. Supernet initialization
% 2. Supernet-based guidance to train edge hypernet (supernet fixed)
% 3. weight hypernet training based on supernet & edge hypernet (supernet & edge hypernet fixed)
% As it is infeasible(?) to jointly train architecture and weights, the conventional strategy for neural architecture search methods is to formulate the search as a bi-level optimization problem~\cite{liu2018darts}, where model weights and architecture are optimized alternately with respect to a fixed training loss.
% In our case, the presence of a preference tuple $(\bm{r},c)$ in the loss function implies solving this expensive optimization procedure for \emph{every} possible preference - this makes the entire process infeasible.


To train our framework, we propose a three stage training procedure.
First, we train a preference agnostic anchor net, which provides the anchor weights at test time (section~\ref{sec:supernet}).
Next, we train the edge hypernet using the prior task relations obtained from the anchor net by optimizing a novel branching regularized loss function derived by inducing a dichotomy over the tasks (section~\ref{sec:hypernet}).
Finally, we train a weight hypernet while fixing the supernet and edge hypernet to adjust the anchor net weights (section~\ref{sec:hypernet}).



\subsection{Network Search Space} \label{sec:search_space}
We utilize a tree-structured network topology which has been shown to be highly effective for multi-task learning in \cite{guo2020learning}. Since tree-structured networks share common low-level features over tasks while extracting task-specific ones in the higher layers, we expect to control the trade-off by learning to change the branching locations conditioned on the desired preference $\left(\bm{r},c\right)$. The search space is represented as a \textit{directed acyclic graph} (DAG), where vertices in the graph represent numerical operations (convolution, pooling etc.) and edges denote the data flow through the network. Figure \ref{fig:block} shows a block of such a graph, containing $N$ \textit{parent} and \textit{child} nodes. The tree-structure is realized by stacking such blocks sequentially and allowing a child node to sample a path from the candidate paths between itself and all its parent nodes. Concretely, the branching operation at layer $l$ can be formulated as $x^{l+1}_j = \mathbb{E}_{d_j\sim p_{\alpha_j^l}} \left[d_j\cdot Y^l\right]$, where $x^{l+1}_j$ denotes the input to the $j$-th node in layer $l+1$, $d_j$ is a one-hot vector indicating the parent node sampled from the \emph{categorical} branching distribution parameterized by $\alpha_j^l$ and, $Y^l = [ y^l_1, \dots, y^l_N ]$ concatenates outputs from all parent nodes at layer $l$
% \begin{equation} \label{eq:branching}
%     x^{l+1}_j = \sum_{j} d_j\cdot y^l_j,
% \end{equation}
% where $x^{l+1}_j$ denotes the input to the $j$-th node in layer $l+1$, $d_j$ is a one-hot vector indicating the parent node sampled from the \emph{categorical} branching distribution parameterized by $\alpha_j^l$ and, \ym{$y^l_i$ is the output of $i^{th}$ node at layer $l$.}
The set of distribution parameters $\bm{\alpha} = \{\alpha_j^l\}_{j \leq N, l < L}$ control the overall structure of the network. This dependence suggests learning these parameters, conditioned on a preference $(\bm{r},c)$, in a manner which satisfies the desired performance trade-off. We describe this learning process in the following sections.

\subsection{Anchor Network} \label{sec:supernet}

In order to simplify the architecture search, we take inspiration from one-shot NAS methods which advocate sharing weights between models via a supernet. Instead of training thousands of separate models from scratch, these methods train a single large supernet capable of emulating any architecture in the search space \cite{bender2018understanding}. Similar to this, we define an \emph{anchor net} which can be not only be used to search for optimal architectures, but also serve as a base network during inference. More specifically, once the anchor net has been trained, architectures can be directly evaluated for their suitability for any preference $(\bm{r},c)$ by inheriting the fixed weights from the anchor net, instead of re-training each time an architecture is chosen for a preference.

% Once the supernet has been trained, architectures can be directly evaluated for their suitability for any preference $(\bm{r},c)$ by inheriting the fixed weights from the supernet, instead of re-training each time an architecture is chosen for a given preference.
% \YM{Supernet has two roles.
% 1) Provide prior of inter-task relationship for training edge hypernet
% 2) Serve as an "anchor network" at test time.
% In the sense that our supernet is used during 'inference' while supernet in one-shot NAS was used for 'training', how about differentiating them by calling our supernet using distinguised name 'anchor net'? And currently, description about 2) seems missing in Method-introduction and not complete in this subsection. So, instead of describing the original supernet ("rather ~ a given preference"), we could replace it to a description of 2).}

% \ym{We aims at initialize the supernet to provide the prior of inter-task relations to guide the edge hypernet.}
We seek to train the anchor net in a manner which provides the prior of inter-task relations to guide the edge hypernet. With this in consideration, as well as the  downstream inference task of dynamic architectural changes, we propose to initialize the anchor net with weights $w^*$, equivalent to a collection of single-task networks as illustrated in Fig.~\ref{fig:framework}(a). This allows sufficient differentiation among individual task streams with distinct features, which was empirically crucial to induce architectural changes in the subsequent stages. While the anchor net trained in such a manner does not capture cross-task edges, it is very effective as: (i) it allows for designing task relationships based on observations in \cite{vandenhende2019branched}, where branching in tree-structured multi-task networks is contingent on how similar task features are at any layer, and (ii) can be further enriched to reflect cross-task edges by the weight hypernet via modulation of normalization parameters.



\subsection{Preference Conditioned Hypernetworks} \label{sec:hypernet}

% Contents to include
% \begin{itemize}
%     \item two separate hypernets (edge + weight): different nature (can be shot as one sentense)
%     \item Hypernetwork input output formulation (originally located at 3.Method intro second paragraph)
%     \item Loss formulation
%     \item (Inference -- already in 3.Method-intro)
% \end{itemize}

%
We employ two hypernetworks to construct our controller for dynamic architectural changes. The edge hypernet $h$, parameterized by $\phi$, predicts the branching parameters $\hat{\bm{\alpha}}=h(\bm{r},c; \phi)$ within the anchor net. On the other hand, the weight hypernet $\bar{h}$, parameterized by $\bar{\phi}$, predicts the normalization parameters $\hat{\bm{\beta},\bm{\gamma}}=\bar{h}(\bm{r},c; \hat{\phi})$ to fine-tune the predicted network. 

We disentangle the training for the two hypernetworks for stability - the edge hypernet is trained first, followed by the weight hypernet. To control the architecture across a wide variety of preferences at the inference time, the hypernetworks should learn to perform architectural changes for a \emph{distribution} $P_{(\bm{r},c)}$ of valid preference vectors rather than a single one. Hence, we adopt a meta-training strategy defined by preferences $\bm{r},c\sim P_{(\bm{r},c)}$, such that the hypernetworks can learn to utilize the relationships between preferences to optimize all of them simultaneously. At test time, when a preference $(\bm{r},c)$ is presented to the controller, the maximum likelihood architecture corresponding to the supplied preference is first sampled from the branching distribution parameterized by the predictions of $h$. Finally, the weights of the tree-structure are inherited from the anchor net, supplemented via adapted normalization parameters predicted by $\bar{h}$. 
\subsubsection{Branching regularized linear scalarization}
To train the edge hypernet, we propose a branching regularized loss function to ensure alignment between the preference and the predicted architecture:
\begin{equation}
    \mathcal{L}_{tot}(\bm{r}) = \mathcal{L}(\bm{r}) + \Omega(\bm{r},c).
\end{equation}

As described previously, $\mathcal{L}(\bm{r})$ denotes the \emph{linear scalarization} of the task specific losses, with the task preference vector $\bm{r}$ as loss weights, i.e. $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$. Optimizing this weighted sum only takes into account the individual task performances without explicitly focusing on the resource allocation within the supernet. In order to control resource allocation, we require a node sharing mechanism which complies with the resource preference $c$ by incorporating the task affinities which implicitly exist in the multi-task learning setup. Consequently, we introduce a branching regularizer $\Omega(\bm{r},c)$ to encourage such node sharing (or branching) based on the preference.
\vskip 2pt
\noindent \textbf{Task Dichotomy.} Depending on the task preferences, we categorise the tasks into two classes. We deem tasks with higher preferences as \textit{active} and those with lower preferences as \textit{inactive}. The former should have a greater influence on the branching structure for an optimal resource-performance trade-off, while the latter may be de-emphasized by encouraging them to follow existing branching choices. To make this distinction concrete, we first define a threshold $\tau$ and then categorise the tasks into active tasks $\mathcal{A}=\{t_i \ | \ r_i \geq \tau, \ \forall i \in [N]\}$, and inactive tasks $\mathcal{I}=\{t_i \ | \ r_i < \tau, \ \forall i \in [N]\}$. The threshold varies with the total number of tasks and is set to values smaller than $1/N$. Based on this classification of tasks, we define two losses, each pertaining to one of the groups, which jointly constitute the regularizer $\Omega(\bm{r},c)$. This explicit emphasizing of certain tasks over others was found to be crucial to induce controllable branching.
\vskip 2pt
\noindent \textbf{Active loss.} We introduce a loss function $\mathcal{L}_{active}$ that encourages nodes in the supernet, corresponding to the active tasks, to be shared in order to avoid the whole network being split up by tasks with little knowledge shared among them. The overall loss is additionally weighted by the resource preference $c$ to control the total resource sharing.  Specifically, we minimize the weighted sum of pairwise $L_2$ distances between the sampled parent edges of the nodes pertaining to the active tasks. Formally, we define $\mathcal{L}_{active}$ as,
\begin{equation} \label{eq:active}
    \mathcal{L}_{active} = c\cdot\sum_{l=1}^L \sum_{\substack{i,j \in \mathcal{A} \\ i\neq j}}
    W(l,i,j)\cdot
    \|\nu^{l}_{i} - \nu^{l}_{j}\|^2,
\end{equation}
where we use the Gumbel-Softmax reparameterization trick~\cite{jang2016categorical} to obtain the samples $\nu^l_i$ from the predicted logits $\hat{\bm{\alpha}}$,
\begin{equation} \label{eq:gumbel}
    \nu^{l}_{i}(k) = \frac{\exp \left((\log \alpha^l_i(k) + G^l_i(k))/\tau\right)}{\sum_{m=1}^N\exp \left((\log \alpha^l_i(m) + G^l_i(m))/\tau\right)}.
\end{equation}
Here, $G^l_i=-\log (-\log U^l_i)$ is a standard Gumbel distribution with $U^l_i$ sampled from a uniform i.i.d. distribution $\text{Unif}(0, 1)$. 

The weight $W(l,i,j)$ in Eqn. \ref{eq:active} reflects how much we want any pair of active tasks to share nodes. We factorize this weight into four components: 
\begin{equation}
    W(l,i,j) = W_{dep}(l) \cdot T_{aff}(i,j) \cdot P_{use}(l,i) \cdot P_{use}(l,j).
\end{equation}

The factor $W_{dep}(l)$ encourages more sharing of nodes which contain low-level features. This is based on the fact that deep networks share low-level features over tasks while extracting task-specific ones in the higher layers, 
\begin{equation}
    W_{dep}(l) = \frac{L-l}{L}
\end{equation}

The factor $T_{aff}(i,j)$ captures the \emph{task affinity} or task relatedness between tasks $\mathcal{T}_i$ and $\mathcal{T}_j$. If two tasks are unrelated, sharing of features can lead to degradation of performance, a phenomenon termed as \emph{negative transfer} \cite{liu2019loss}. To this end, we base the layer sharing on measurable levels of task affinity: two tasks are strongly related, if their single task models rely on a similar set of features. We adopt \emph{Representational Similarity Analysis} (RSA)~\cite{dwivedi2019representation} to obtain the task affinity scores from the anchor net. The formulations are detailed in the supplementary material.

The two final factors ensures that the loss is applied correctly to only the nodes which are a part of the sampled architecture (has a connection to the leaf nodes). The factor $P_{use}(l,i)$ represents the probability that the node $i$ at layer $l$ is present in the tree structure that is sampled by the hypernetwork. We follow a dynamic programming approach to calculate this value. Denoting the $i^{th}$ node in the $l^{th}$ layer as $(l,i)$, we can define the marginal probability that the node $(l+1,k)$ samples the node $(l,i)$ as its parent as $\nu^{l}_k(i)$.  Thus, the probability that the node $(l,i)$ is used in the sampled tree structure is
\ym{
\begin{equation}
    P_{use}(l,i)
    = 1 - \prod_{k}\{ 1 - P_{use}(l+1,k) \cdot \nu^{l}_k(i) \},
    % = 1 - \prod_{k}\{ 1 - P_{use}(l+1,k)P_{par}(l, i \rightarrow k) \},
    % = \sum_{j} { P_{par}(l, i \rightarrow j) P_{use}(l+1, j)},
\end{equation}
where $P_{use}(L,i) = 1$ for all $i \in [N]$.}
\vskip 2pt
\noindent \textbf{Inactive loss.} 
The inactive tasks should have minimal effect in terms of branching. To encourage this behavior, we introduce $\mathcal{L}_{inactive}$ to encourage these tasks to mimic the most closely related branching pattern, 
\begin{equation}
    \mathcal{L}_{inactive} = \sum_{l} \sum_{j \in \mathcal{I}}
     \min_{i \in \mathcal{A}} \|\nu^{l}_{i} - \nu^{l}_{j}\|^2.
\end{equation}
This ensures that the network branching is controlled by the active tasks, with the inactive tasks sharing nodes with the active tasks.

Thus, the branching regularizer is defined as follows,
\begin{equation}
    \Omega(\bm{r},c) = \lambda_{\mathcal{A}}\mathcal{L}_{active} + \lambda_{\mathcal{I}}\mathcal{L}_{inactive},
\end{equation}
where $\lambda_{\mathcal{A}}$, $\lambda_{\mathcal{I}}$ are hyperparameters to determine the weighting of the losses. Typically, we set $\lambda_{\mathcal{A}}=0.05$ and $\lambda_{\mathcal{I}}=0.1$.


\subsubsection{Cross-task adaptation}
The architecture sampled by the edge hypernet $h$ contains edges which have not been observed during the anchor net training. We denote these as \emph{cross-task} edges since these connect nodes belonging to different streams in the anchor net. Consequently, the performance of the sampled network is sub-optimal. To rectify this issue, we propose to fine-tune the weights of the anchor net to adapt it these unseen edges using an additional weight hypernet $\bar{h}$. 

Since the anchor net parameters can be high dimensional, tuning all the weights is highly sensitive and inefficient. As an alternative to fine-tuning all the model’s parameters, prior work \cite{wang2020tent,mahabadi2021parameter} estimates normalization statistics and optimizes channel-wise affine transformations. Following suit, we propose to generate normalization parameters using a hypernetwork in order to capture the cross-task information to enhance the final performance.

Conventional batch normalization at layer $l$ for node $i$ is defined as,
\begin{align}
    \text{BN}_i^l(\bm{x}^l_i) = \gamma^l_i\frac{x^l_i-\mu^l_{i}}{\sigma_i^l} + \beta^l_i,
\end{align}
where $\gamma^l_i$ and $\beta^l_i$ are the learnable parameters, and $\mu^l_i$ and $\sigma^l_i$ denote the batch statistics of the node input $x^l_i$. Given a preference $(r,c)$ and predicted branching parameters $\hat{\bm{\alpha}}=h(\bm{r},c; \phi)$, we predict perturbations to the batch normalization parameters using $\bar{h}$: $\{\Delta \gamma^l_i,\Delta \beta^l_i\}_{i \leq N, l < L} = \bar{h}(r,c;\theta)$. This allows us to redefine the batch normalization layers as follows, 
\begin{align}
    \text{BN}_i^l(\bm{x}^l_i) = (\gamma^l_i+\Delta\gamma^l_i)\frac{x^l_i-\mu^l_{i}}{\sigma_i^l} + (\beta^l_i+\Delta\beta^l_i).
\end{align}

We train $\bar{h}$ by first sampling preferences $\bm{r},c\sim P_{(\bm{r},c)}$ and the architecture from the edge hypernet $h$, and then applying the predicted normalization parameter perturbations along the sampled architecture to optimize the linear scalarized task losses $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$.

% The architecture sampled by the hypernetwork $h$ contains edges which have not been observed during the supernet training. We denote these as \emph{cross-task} edges in relation to the fact that these edges connect nodes belonging to different tasks in the supernet. Consequently, the performance of the sampled network is sub-optimal. To rectify this issue, we need to fine-tune the weights of $F$ to adapt it these unseen edges. In order to preserve the online nature of our framework we use an additional hypernetwork $\bar{h}$ to predict the fine-tuned weights of the architecture sampled by $h$. 

% However, $F$ is non-linear and its parameters can be high dimensional, making optimization too sensitive and inefficient for online prediction. As an alternative to fine-tuning all the model’s parameters, prior work \cite{wang2020tent} estimates normalization statistics and optimizes channel-wise affine transformations. Following suit, we propose to generate normalization parameters using a hypernetwork in order to capture the cross-task information to enhance the final performance.

% Conventional batch normalization at layer $l$ for node $i$ is defined as,
% \begin{align}
%     \text{BN}_i^l(\bm{x}^l_i) = \gamma^l_i\frac{x^l_i-\mu^l_{i}}{\sigma_i^l} + \beta^l_i,
% \end{align}
% where $\gamma^l_i$ and $\beta^l_i$ are the learnable parameters, and $\mu^l_i$ and $\sigma^l_i$ denote the batch statistics of the node input $x^l_i$. Given a preference $(r,c)$ and predicted branching parameters $\hat{\bm{\alpha}}=h(\bm{r},c; \phi)$, we predict perturbations to the batch normalization parameters using $\bar{h}$: $\{\Delta \gamma^l_i,\Delta \beta^l_i\}_{i \leq N, l < L} = \bar{h}(r,c;\theta)$. This allows us to redefine the batch normalization layers as follows, 
% \begin{align}
%     \text{BN}_i^l(\bm{x}^l_i) = (\gamma^l_i+\Delta\gamma^l_i)\frac{x^l_i-\mu^l_{i}}{\sigma_i^l} + (\beta^l_i+\Delta\beta^l_i).
% \end{align}

% We train $\bar{h}$ by first sampling preferences $\bm{r},c\sim P_{(\bm{r},c)}$ and the architecture from the hypernetwork $h$ trained previously, and then apply the predicted normalization parameter perturbations along the sampled architecture to optimize the linear scalarized task losses $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$.

% \XY{A bit confused on Section 3 and Section 5. Maybe you are looking into which one is better for method. I'll look into it after it is fixed.}
\subsection{Implementation Details} \label{sec:implementation_details}
% input token (use token, instead of directly putting into fc)
% network details (supernet, hypernets)
% training params

==> sections/method_old.tex <==

\section{Method}

Given a set of $N$ tasks $\bm{T}=\{\mathcal{T}_1,\mathcal{T}_2,\dots,\mathcal{T}_N\}$, most multi-task learning algorithms focus on learning the weights of a model (and architecture) to minimize a weighted sum of several loss terms: $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$, where each $\mathcal{L}^i$ represents the loss associated with task $\mathcal{T}_i$, and $\bm{r} \in \mathcal{S}_N$, with $\mathcal{S}_N=\{\bm{r}\in\mathbb{R}^N | \sum_i r_i = 1, r_i \geq 0\}$ representing the $N$-dimensional simplex~\cite{ruder2017overview}. Here, $\bm{r}$ denotes a preference vector signifying the desired trade-off over the different tasks. Typically, one minimizes the loss independently for each choice of the preference vector $\bm{r}$. In contrast, we propose a framework which can approximate the entire trade-off curve for the multi-task problem, in terms of \emph{model architecture}, using a \textit{single} model. More precisely, we utilize a \textit{hypernetwork}~\cite{ha2016hypernetworks}, which takes as input a preference $\bm{r}$ to dynamically allocate model resources over the tasks in proportion to the supplied preference.

We introduce the network design space for dynamic architecture search in Section \ref{sec:search_space}.
%\YM{specify output format? which is specified by the choice of parent node for every node} Inspired by one-shot neural architecture search methods, our training scheme consists of two stages. 
A preference agnostic supernet is trained first to enforce task priors,
as outlined in Section \ref{sec:supernet}. This is subsequently used in the second stage of training by the hypernetworks, which are described in Section \ref{sec:hypernet}.

\subsection{Network Search Space} \label{sec:search_space}
To perform dynamic architectural changes, we need to first define a search space which can represent a wide variety of architectures. In this work, we utilize a tree-structured network topology which has been shown to be highly effective for multi-task learning in \cite{guo2020learning, bruggemann2020automated}.
Since tree-structured networks share common low-level features over tasks while extracting task-specific ones in the higher layers, we expect to control the trade-off by learning to change the branching locations conditioned on the preference $\bm{r}$.

The search space is represented as a \textit{directed acyclic graph } (DAG), where vertices in the graph represent numerical operations (convolution, pooling etc.) and edges denote the data flow through the network. Figure \ref{fig:block} shows a block of such a graph, containing $N$ \textit{parent} and \textit{child} nodes. The tree-structure is realized by stacking such blocks sequentially and allowing a child node to sample a path from the candidate paths between itself and all its parent nodes. Concretely, the branching operation at layer $l$ can be formulated as:
\begin{equation} \label{eq:branching}
    x^{l+1}_j = \mathbb{E}_{d_j\sim p_{\alpha_j^l}} \left[d_j\cdot Y^l\right]
\end{equation}
where $x^{l+1}_j$ denotes the input to the $j$-th node in layer $l+1$, $d_j$ is a one-hot vector indicating the parent node sampled from the \emph{categorical} branching distribution parameterized by $\alpha_j^l$ and, $Y^l = [ y^l_1, \dots, y^l_N ]$ concatenates outputs from all parent nodes at layer $l$.
The set of distribution parameters $\bm{\alpha} = \{\alpha_j^l\}_{j \leq N, l \leq L}$ control the overall structure of the network. This dependence suggests learning these parameters, conditioned on a preference vector $\bm{r}$, in a manner which satisfies the desired performance trade-off. We describe this learning process in the following sections.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{images/branching_block.pdf}
    \caption{\textbf{Branching block.} Illustration of the parent sampling operation from Eqn. \ref{eq:branching}. Nodes in layer \textcolor{blue}{$l$} are sampled in accordance to a categorical distribution for each node in layer \textcolor{red}{$l+1$}.}
    \label{fig:block}
\end{figure}

\subsection{Initialization via Weight-Sharing} \label{sec:supernet}
% \YM{Conventional strategy for neural architecture search is to formulate the problem as a bi-level optimization. It seeks optimal network architecture that minimizes objective computed from optimal weights found in the first-level optimization given the architecture~\cite{}}.

The conventional strategy for neural architecture search methods is to formulate the search as a bi-level optimization problem~\cite{liu2018darts},
\begin{equation}
\begin{split}
    & \min_{\bm{\alpha}} \ \mathcal{L}\left(w^*(\bm{\alpha}), \bm{\alpha}\right) \\ 
    & \text{s.t.} \ w^*(\bm{\alpha}) = \min_{w} \ \mathcal{L}\left(w,\bm{\alpha}\right)
\end{split}
\end{equation}
% \YM{formulation for our problem?}
where $w$ represents the model weights, $\bm{\alpha}$ determines the network architecture and $\mathcal{L}$ denotes the training loss. In our case, the presence of a preference vector $\bm{r}$ implies solving this expensive optimization procedure for \emph{every} possible preference, which makes the entire process computationally infeasible.

% \YM{as this is to motivate 2-stage training, add explanation of hypernet to explain how $\bm{r}$ adds additional layer of complexity?}
% \YM{
% \begin{align}
% \min_{\phi, \psi} \mathbb{E}_{\mathbf{r}}[L_{\mathbf{r}}(\alpha, w)] \\
% \text{where } \alpha = \Phi(\mathbf{r}, \phi), w = \Psi(\mathbf{r}, \psi)
% \end{align}
% }

In order to simplify the problem, we take inspiration from one-shot neural architecture search methods which advocate sharing weights between models by training a \textit{supernet}: rather than training thousands of separate models from scratch, one can train a single large network capable of emulating any architecture in the search space \cite{bender2018understanding}. Once the supernet has been trained, architectures can be directly evaluated for their suitability for any preference $\bm{r}$ by inheriting the weights from the supernet, instead of re-training each time for some architecture chosen for a preference $\bm{r}$.

With the downstream task of dynamic architectural changes in consideration, we propose to compose the supernet $F$ as a collection of single-task networks. In terms of the parent-child blocks defined in the previous section, the branching distribution parameters are defined as:
\begin{equation}
    \alpha_j^l = \mathbf{e}_j, \ \forall \  j \in [N], \  l \in [L]  
\end{equation}
where $\mathbf{e}_j$ denotes the $j$-th standard basis vector of $\mathbb{R}^N$ (see Figure \ref{fig:supernet}). Thus, node $j$ in any layer corresponds to the the task $t_j$.
% \YM{in the previous definition, $\alpha$ parameterize $P_{\alpha}$ but function is not defined yet}
Using this fully branched structure, the supernet weights are trained to minimize the following loss:
\begin{equation}
    \mathcal{L}_{sup} = \sum_{i=1}^N\mathcal{L}^i
\end{equation}
At the conclusion of training, we obtain the optimal weights $w^*$ of the supernet $F$. Note that the training of the supernet is completely preference agnostic, and serves solely to provide a prior for the subsequent stage. 

We motivate our supernet training strategy via observations in \cite{vandenhende2019branched}, whereby branching in multi-task networks is contingent on task affinity: two tasks are strongly related, if their single task models rely on a similar set of features and vice versa. In other words, pre-trained single task networks provide sufficient information for learning the branching distribution parameters. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/supernet.pdf}
    \caption{\textbf{Supernet training.} We compose the supernet as a collection of single task networks, with each task stream shown in a  different colour ($(l,i)$ represents the $i$-th node in layer $l$).}
    \label{fig:supernet}
\end{figure}

\subsection{Preference Conditioned Hypernetworks} \label{sec:hypernet}

As described in Section \ref{sec:search_space}, every possible architecture in consideration is described concisely by the set of branching parameters $\bm{\alpha}$. Since the number of potential configurations grows exponentially with the number of layers and tasks, it becomes intractable to manually find the optimal architecture for every possible preference vector.
\YM{complexity grows exponentially with the number of tasks?}
Thus, we propose to use hypernetworks \cite{ha2016hypernetworks} to sample optimal tree-structured architectures from the supernet to satisfy the given task preferences. \footnote{Note that when we mention that the hypernetwork samples architectures, we wish to convey that it predicts the parameters of the branching distributions from which we sample the tree structures. We follow this for conciseness.}

Concretely, we train a hypernetwork $h$, parameterized by $\phi$, to predict the branching parameters $\hat{\bm{\alpha}}_{\bm{r}}=h(\bm{r}; \phi)$ within the supernet $F$. Since we wish to control the resource allocation at the inference time, the hypernetwork should learn to perform architectural changes for a \emph{distribution} $P_{\bm{r}}$ of valid preference vectors rather than a single one. Hence, during training time the model observes many losses, defined by preferences $\bm{r}\sim P_{\bm{r}}$, and can
learn to utilize the relationships between them to optimize all of them simultaneously. At test time, when a preference $\bm{r}$ is presented to the hypernetwork, the optimal tree-structure corresponding to $\bm{r}$ is sampled from the branching distribution parameterized by the predictions of $h$, and is used directly for inference in the supernet $F$. 

\subsubsection{Branching regularized linear scalarization}
To ensure alignment between the preference and the architecture predicted by the hypernetwork, we propose a branching regularized loss function to train the hypernetwork:
\begin{equation}
    \mathcal{L}_{tot}(\bm{r}) = \mathcal{L}(\bm{r}) + \Omega(\bm{r}).
\end{equation}
As described previously, $\mathcal{L}(\bm{r})$ denotes the \emph{linear scalarization} of the task specific losses, with the preference vector $\bm{r}$ as loss weights, i.e. $\mathcal{L}(\bm{r}) = \sum_ir_i\mathcal{L}^i$. Optimizing this weighted sum only takes into account the individual task performances without explicitly focusing on the resource allocation within the supernet. However, we seek compact tree-structures in which nodes are shared as much as possible, based on the task affinities which implicitly exist in the multi-task learning setup, without deteriorating the task performance. Consequently, we introduce a branching regularizer $\Omega(\bm{r})$ to encourage such node branching (or sharing) based on $\bm{r}$.

\textbf{Task dichotomy.} The core hypothesis that underlies the design of the branching regularizer is that \emph{not all tasks influence the branching structure equally}. Given a preference vector $\bm{r}$, the resulting branching pattern should be dominated by tasks with preference values which are above a certain threshold. We denote such tasks as \emph{active} tasks. The remaining tasks are referred to as \emph{inactive} tasks. We denote the set of active tasks as $\mathcal{A}=\{t_i \ | \ r_i \geq \gamma, \ \forall i \in [N]\}$, while the inactive tasks are represented similarly,  $\mathcal{I}=\{t_i \ | \ r_i < \gamma, \ \forall i \in [N]\}$. Here $\gamma$ is a hyperparameter which defines the threshold. Based on this classification of tasks, we define two losses, each pertaining to one of the groups, which jointly constitute the branching regularizer $\Omega(\bm{r})$. 

\textbf{Active loss.} We introduce a loss function $\mathcal{L}_{active}$ that encourages nodes in the supernet, corresponding to the active tasks, to be shared in order to avoid the whole network being split up by tasks with little knowledge shared among them. Specifically, we minimize the weighted sum of pairwise $L_2$ distances between the sampled parent edges of the nodes pertaining to the active tasks. Formally, we define $\mathcal{L}_{active}$ as,
\begin{equation} \label{eq:active}
    \mathcal{L}_{active} = \sum_{l} \sum_{\substack{i,j \in \mathcal{A} \\ i\neq j}}
    W(l,i,j)\cdot
    \|\nu^{l}_{i} - \nu^{l}_{j}\|^2,
\end{equation}
where we utilize the Gumbel-Softmax reparameterization trick \cite{} to obtain the samples $\nu^l_i$ from the predicted logits $\alpha^l_i$.
The weight $W(l,i,j)$ in Eqn. \ref{eq:active} reflects how much we want any pair of active tasks to share nodes. We factorize this weight into four components: 
\begin{equation}
    W(l,i,j) = P_{use}(l,i) \cdot P_{use}(l,j) \cdot W_{dep}(l) \cdot T_{rel}(i,j) .
\end{equation}

\YM{Can we add another figure that shows $alpha$s in the layers to help interpreting notations?}

The factor $P_{use}(l,i)$ represents the probability that the node $i$ at layer $l$ is present in the tree structure that is sampled by the hypernetwork. We follow a dynamic programming approach to calculate this probability. Let us denote the $i^{th}$ node in the $l^{th}$ layer as $(l,i)$. We can define the marginal probability that the node $(l+1,k)$ samples $(l,i)$ as its parent as,
\begin{equation}
    P_{par}(l, i \rightarrow k)
    = \frac{\exp\left(\alpha^{l+1}_{k}(i)\right)}
      {\sum_{z}{\exp\left(\alpha^{l+1}_{k}(z)\right)}}.
\end{equation}
Thus, the probability that the node $(l,i)$ is used in the sampled tree structure is
\begin{align}
    P_{use}(l,i)
    = 1 - &\prod_{k}\{ 1 - P_{use}(l+1,k)P_{par}(l, i \rightarrow k) \}
    % = \sum_{j} { P_{par}(l, i \rightarrow j) P_{use}(l+1, j)},
\end{align}
where
\begin{align}
    P_{use}(L-1,i)
    &= 1 - \prod_{k} \left(1 - P_{par}(L-1, i \rightarrow k)\right) \nonumber \\
    &= 1 - \prod_{k} \left(1 - \frac{\exp\left(\alpha^{L}_{k}(i)\right)}
                              {\sum_{z}{\exp\left(\alpha^{L}_{k}(z)\right)}}\right).
\end{align}

The factor $W_{dep}(l)$ encourages more sharing of nodes which contain low-level features. This is based on the fact that deep networks share low-level features over tasks while extracting task-specific ones in the higher layers, 
\begin{equation}
    W_{dep}(l) = \frac{L-l}{L}
\end{equation}

The final factor $T_{rel}(i,j)$ captures the \emph{task affinity} or task relatedness between tasks $t_i$ and $t_j$. If two tasks are unrelated, sharing of features can lead to degradation of performance, a phenomenon termed as \emph{negative transfer} \cite{}. To this end, we base the layer sharing on measurable levels of task affinity: two tasks are strongly related, if their single task models rely on a similar set of features. We adopt \emph{Representational Similarity Analysis} (RSA) \cite{} to obtain the task affinity scores from the supernet $F$. First, using a subset of $K$ instances, we extract the features for each of these data points for every task. Let us denote the extracted feature for instance $k$ at layer $l$ for task $t_i$ as $\bm{f}_{[i,l,k]}$. Using these features, we compute the feature dissimilarity tensor $\mathbf{D}_l$ at each layer, of dimensions $N\times K \times K$, as follows,
\begin{equation}
    \mathbf{D}_l \left(i,j,k\right) = 1 - \frac{\langle\bm{f}_{[i,l,j]},\bm{f}_{[i,l,k]}\rangle}{\|\bm{f}_{[i,l,j]}\|\|\bm{f}_{[i,l,k]}\|}.
\end{equation}
The task affinity matrix $\bm{T}_l$ at layer $l$, of dimensions $N \times N$, is calculated as follows,
\begin{equation}
    \bm{T}_l(i,j) = \|\mathbf{D}_l \left(i,:,:\right)-\mathbf{D}_l \left(j,:,:\right)\|_{F}.
\end{equation}
The factor $T_{rel}(i,j)$ is obtained by taking the mean of the affinity scores across layers, i.e., $T_{rel}(i,j)=\frac{1}{L}\sum_l\bm{T}_l(i,j)$.

\textbf{Inactive loss.} 
As discussed previously, the inactive tasks should have minimal effect in terms of branching. To enforce this, we introduce $\mathcal{L}_{inactive}$ to encourage these tasks to mimic the most closely related branching pattern, 
\begin{equation}
    \mathcal{L}_{inactive} = \sum_{l} \sum_{j \in \mathcal{I}}
     \min_{i \in \mathcal{A}} \|\nu^{l}_{i} - \nu^{l}_{j}\|^2.
\end{equation}


% - weighted loss and branching \\
% - active/inactive tasks \\
% - active loss \\
% - inactive loss \\
% - task similarity computation

% \subsubsection{Hypernetwork for cross-connections adaptation}




% \paragraph{Hypernetwork for edge prediction} \mbox{}\\
% - task similarity matrix computation \\
% - linear scalarization \\
% - branching losses 
% \paragraph{Hypernetwork for cross-connections adaptation}

% \paragraph{Algorithm} \mbox{}\\






% Consider a supernet that consists of $T$ streams for $T$ tasks.
% Each stream consists of $L$ sequential modules where $L^{th}$ layer corresponds to the task-specific head.
% Let us denote the $i^{th}$ node in the $l^{th}$ layer as $(l,i)$.
% % To simplify notation, we denote the input image as the node of the $0^{th}$ layer.
% At each trial, each node independently samples its parent node.
% Once every node selects its parent, the network architecture is specified to the corresponding tree structure.
% Note that different combinations of parent selections can havet the same tree structure.
% %For example,

% We define the marginal probability that the node $(l+1,j)$ choose $(l,i)$ as its parent as
% \begin{equation}
%     P_{par}(l, i \rightarrow j)
%     = \frac{\exp(\alpha^{l+1}_{j,i} / \tau)}
%       {\sum_{k}{\exp(\alpha^{l+1}_{j,k} / \tau)}}.
% \end{equation}
% % Here, $\alpha^{l}_{i,j}$ is a scalar.
% The sample space is the set of all possible combinations of parent selections as shown in Figure~\ref{fig:sample_space}.
% The probability that the node $(l,i)$ is used in the tree structure is
% \begin{align}
%     P_{use}(l,i)
%     = 1 - &\prod_{j}\{ 1 - P_{use}(l+1,j)P_{par}(l, i \rightarrow j) \}
%     % = \sum_{j} { P_{par}(l, i \rightarrow j) P_{use}(l+1, j)},
% \end{align}
% where
% \begin{align}
%     P_{use}(L-1,i)
%     &= 1 - \prod_{j} (1 - P_{par}(L-1, i \rightarrow j)) \nonumber \\
%     &= 1 - \prod_{j} (1 - \frac{\exp(\alpha^{L}_{j,i} / \tau)}
%                               {\sum_{k}{\exp(\alpha^{L}_{j,k} / \tau)}}).
% \end{align}


% Active loss is formulated as
% \begin{equation}
%     L_{act} = \sum_{l} \sum_{\substack{i,j \\ i\neq j}}
%     P_{use}(l,i) P_{use}(l,j)
%     % (\sum_{t \in \mathcal{A}} P_{task}(l,i,t))
%     % (\sum_{t \in \mathcal{A}} P_{task}(l,j,t))
%     \|\alpha^{l}_{i,\cdot} - \alpha^{l}_{j,\cdot}\|^2,
% \end{equation}
% where
% % $\mathcal{A}$ is the set of active tasks and 
% $\alpha^l_{i,\cdot} = [\alpha^l_{i,1}, \cdots, \alpha^l_{i,t}]\in \mathbb{R}^T$.

% Inactive loss is formulated as
% {\color{red}
% \begin{equation}
%     L_{inact} = \sum_{l} \sum_{j}
%     (1 - P_{use}(l,j))
%      \min_{i} P_{use}(l,i) \|\alpha^{l}_{i,\cdot} - \alpha^{l}_{j,\cdot}\|^2,
% \end{equation}
% }

% The expected number of used nodes in the tree structure is
% \begin{equation}
%     \sum_{l,i} P_{use}(l,i).
% \end{equation}

% \ym{scalability}

==> tables/flops.tex <==
\begin{table}[h]
\centering
% \footnotesize
\resizebox{0.75\columnwidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{GFLOPS}} \\
\multicolumn{1}{c}{}                        & Pascal (5 tasks)    & Pascal (3 tasks)  & NYU-v2    \\ \midrule
Single-Task                               
& 16.17                  
& 9.75
& 58.78\\
Multi-Task     
& 6.28                
& 4.81
& 21.02\\
Ours, c=0.0  
& 7.21                  
& 5.52
& 29.04\\
Ours, c=1.0  
& 6.81                   
& 5.07
& 25.98\\\bottomrule
\end{tabular}%
}
\vspace{-0.6cm}
\label{tab:flops}
\end{table}

==> tables/multitask.tex <==
\begin{table}[h]
\centering
\footnotesize
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}cccc@{}}
\toprule
Pascal (3) & Pascal (5) & NYU-v2 & CIFAR-100 \\ \midrule
4.02           & 69.02            & 11.93       & 0.007          \\ \bottomrule
\end{tabular}%
}
\vspace{-0.42cm}
\end{table}

==> tables/nyu_3task_2.tex <==
\begin{table}[]
\label{tab:pascal3_arch}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{l}{\textbf{Method}} & \multicolumn{1}{c}{$\Delta_{\mathcal{T}_1} \uparrow$} & \multicolumn{1}{c}{$\Delta_{\mathcal{T}_2} \uparrow$} & \multicolumn{1}{c}{$\Delta_{\mathcal{T}_1} \uparrow$} & \multicolumn{1}{c}{$\Delta_{\mathbf{T}} \uparrow$} & \# \textbf{Params} (\%) $\downarrow$                  \\ \midrule
LTB                        & -20.35  & -13.65  & -5.17  & -13.06   & \textbf{-51.2}    \\ \midrule 
Ours, c=0.0                & \textbf{0.0 }                    & \textbf{+0.90}                & \textbf{+3.44}                  & \textbf{+1.45}                     & -10.4                     \\ 
$\text{Ours}^\dagger$, c=0.0                & -0.58                 & +0.45                  & +3.44                  & +1.10                     & -10.4                     \\
Ours, c=1.0                & -0.88                 & 0.0                     & 0.0                     & -0.29                    & -22.1 \\

$\text{Ours}^\dagger$, c=1.0                & -1.17                 & -0.45                 & 0.0                     & -0.54                    & -22.1                    \\ \bottomrule
\end{tabular}}
\caption{\textbf{Architecture evaluation on NYU-v2}}
\end{table}

==> tables/preference.tex <==
\begin{table}[h!]
\small
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{lllll}
\toprule
$\eta$   & 0.1 & 0.2 & 0.5 & 1.0 \\ \midrule
c=0.0 &4.20     &4.25     &4.26     &4.26     \\
c=1.0 &4.18     &4.26     &4.25     &4.21     \\ \bottomrule
\end{tabular}%
% }
\vspace{-0.42cm}
\end{table}
